COKE: A Cognitive Knowledge Graph for Machine Theory of Mind

Theory of mind (ToM) refers to humans' ability to understand and infer the desires, beliefs, and intentions of others. The acquisition of ToM plays a key role in humans' social cognition and interpersonal relations. Though indispensable for social intelligence, ToM is still lacking for modern AI and NLP systems since they cannot access the human mental state and cognitive process beneath the training corpus. To empower AI systems with the ToM ability and narrow the gap between them and humans, in this paper, we propose COKE: the first cognitive knowledge graph for machine theory of mind. Specifically, COKE formalizes ToM as a collection of 45k+ manually verified cognitive chains that characterize human mental activities and subsequent behavioral/affective responses when facing specific social circumstances. In addition, we further generalize COKE using LLMs and build a powerful generation model COLM tailored for cognitive reasoning. Experimental results in both automatic and human evaluation demonstrate the high quality of COKE, the superior ToM ability of COLM, and its potential to significantly enhance social applications.

==> sections/00-abstract.tex <==
Theory of mind (ToM) refers to humans' ability to understand and infer the desires, beliefs, and intentions of others. 
The acquisition of ToM plays a key role in humans' social cognition and interpersonal relations.
Though indispensable for social intelligence, ToM is still lacking for modern AI and NLP systems since they cannot access the human mental state and cognitive process beneath the training corpus.
To empower AI systems with the ToM ability and narrow the gap between them and humans, in this paper, we propose \cokewithemoji: the first cognitive knowledge graph for machine theory of mind. Specifically, \coke formalizes ToM as a collection of 45k+ manually verified cognitive chains that characterize {human mental activities} and subsequent behavioral/affective responses when facing specific {social circumstances}. 
Beyond that, we further generalize \coke using pre-trained language models and build a powerful generation model \cokelm tailored for cognitive reasoning.
% build a powerful cognitive generation model \cokelm.
Experimental results in both automatic and human evaluation demonstrate the high quality of \coke and the superior ToM ability of \cokelm.

==> sections/01-introduction.tex <==
\section{Introduction}
% \footnote{1 Our data and codes will be available at }
% 人类在社交过程中，不仅需要理解其他人正在做的事，还要预测他们将要做的事，这就是Theroy of Mind. citeToM原始论文。
In social environments, human beings must be able not only to react to what others are doing, but also to anticipate what they will do. This ability to understand and infer human goals is typically described as our Theory of Mind (ToM) \cite{premack1978tom}.
% 一种ToM的实现方式就是观察别人在特定社交场景下所做的事，并总结出一套情感和行为的规则。当相同或相似的事情发生时，我们就可以进行情感和行为的预测。cite 30year 论文
One way of accomplishing ToM is to observe what others do in various situations, and derive a set of affective and behavioral rules.
% and then predict what others will do in a specific situation \cite{call2011tom30year}. 
When the same or highly similar things arise again, we can bring out plausible predictions accordingly \cite{call2011tom30year}.
% 对于人类而言，我们在生长发育的过程中逐渐建立了对ToM的认知。
%For humans, the establishment of ToM begins in our childhood and continues throughout our entire life \cite{giovagnoli2019tomage}.
%例如，我们可以完成以下的认知过程：当一个研究者正在完成一篇论文时，如果deadline很接近了，他很可能会认为无法完成工作，感觉压力很大，并熬夜工作。当一个研究者在完成一篇即将overdue的论文时，我们推测他很可能会觉得stressed-out(affective reaction)并会stay up late to work(behavior reaction)。
%For example, according to our life experience, we can complete the following cognitive process of ToM. When a researcher is finishing a paper (a specific situation), if the deadline is very close, he is likely to think that the work cannot be completed, feel stressed (an affective prediction), and stay up late to work(a behavioral prediction). 
Figure \ref{fig-intro} presents an example that \emph{someone will deliver a talk at the university tomorrow} (a social circumstance), and \emph{he has substantial public speaking experience} (a trigger factor). We can plausibly anticipate that \emph{he will deliver an impressive speech} (a mental activity), \emph{feels joyful} (an affective response), and \emph{has a restful sleep tonight} (a behavioral response). Here ToM is instantiated as a chained cognitive process that derives from our knowledge, experiences, and memories \cite{harris1989young}.
%When a researcher is finishing a paper that is about to be overdue, we speculate that he will probably feel stressed-out (an affective prediction) and will stay up late to work (a behavioral prediction).
% ToM对于人类社会至关重要，因为它使得我们可以在没有omniscient and omnipotent visual angle时，leverage our own minds to simulate others',从而实现efficient和effective communication.
ToM is indispensable to humans since it allows us to leverage our own minds to simulate others', so as to achieve efficient communication \cite{RabinowitzPSZEB18}.
% \begin{figure}[t]
% 	\centering
% 	\vspace{0mm}
% 	\hspace{0mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	\includegraphics[width=0.98\linewidth]{figures/intro}
% 	\centering
% 	\caption{An illustration of the proposed \coke framework to monitor the machine theory of mind.}
% 	\label{fig-intro}
% 	\vspace{-5mm}
% \end{figure}

\begin{comment}
\begin{figure}[t]
	\centering
	\vspace{0mm}
        % \vspace{-10mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
        % \includegraphics[width=0.98\linewidth]{figures/intro_case.png}
	% \includegraphics[width=0.98\linewidth]{figures/intro_case3.png}
        %\includegraphics[width=0.50\textwidth]{figures/intro_c.png}
        % \includegraphics[width=0.50\textwidth]{figures/intro_cz}
    \includegraphics[width=0.98\textwidth]{figures/intro_cz}
	\centering
	\caption{\coke instantiates the Theory of Mind as cognitive chains in social situations.}
	\label{fig-intro}
	\vspace{-7mm}
\end{figure}    
\end{comment}

\begin{figure}[t]
	\centering
	\vspace{0mm}
	% \hspace{0mm}
        \hspace{0mm}
	\setlength{\abovecaptionskip}{0mm}
	\setlength{\belowcaptionskip}{0mm}
 %        \includegraphics[width=0.98\linewidth]{figures/intro_case.png}
	% \includegraphics[width=0.98\linewidth]{figures/intro_case3.png}
 %        \includegraphics[width=0.50\textwidth]{figures/intro_c.png}
        \includegraphics[width=0.46\textwidth]{figures/intro_cz}
	\centering
	\caption{\coke instantiates Theory of Mind as positive and negative cognitive chains in social situations.}
	\label{fig-intro}
	\vspace{-7mm}
\end{figure}

% \begin{figure*}[h]
% 	\centering
% 	\vspace{-10mm}
% 	\hspace{-3mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	\includegraphics[width=0.9999\linewidth]{figures/dimension}
% 	\centering
% 	%\caption{An overview of five types of nodes and their definitions in \coke.}
% 	\caption{ \coke instantiates Theory of Mind as cognitive chains containing five types of nodes.}

% 	\label{fig-intro}
% 	\vspace{-4mm}
% \end{figure*}

% 然而，现代NLP系统(如预训练语言模型)虽然具有强大的语言建模和生成能力，但却没有well equipped with ToM.
Despite its importance for social intelligence, ToM is not well internalized by modern AI and NLP systems. 
%(e.g., pre-trained language models). 
%Although being powerful in language understanding and generation, NLP systems are usually trained by explicit human-generated corpus and 
%However, modern NLP systems (such as pre-trained language models) are not well equipped with ToM despite their powerful language modeling and generation capabilities.
% 主要原因在于，NLP系统通常由human表达的显式自然语言文本训练，而不能have access to the latent cognitive process and mental states of humans. cite
The main reason is that learning-based systems are usually trained on superficial text corpus, while 
% they have no
lacking access to the underlying human mental state and cognitive process \cite{Sap2022NeuralTO}.  
%从而，NLP系统依赖于maximum likelihood对人类的affective和behavior进行理解和生成，而非基于the theory of mind.
In other words, NLP systems rely on the maximum likelihood to understand and generate texts, but do not go beneath the surface to the desires, beliefs, and intentions of humans.
\begin{figure*}[t]
	\centering
	\vspace{0mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	\includegraphics[width=0.90\linewidth]{figures/dimension}
	\centering
	\caption{An overview of five types of nodes and their definitions in \coke.}
	\label{fig-dimension}
	\vspace{-4mm}
\end{figure*}
In this paper, we introduce \cokewithemoji: the first \emph{\textbf{CO}gnitive \textbf{K}nowledg\textbf{E} graph} for machine theory of mind. Our goal is to formalize ToM and make it accessible and learnable for AI systems. In \coke, we instantiate ToM as a collection of manually verified cognitive chains that characterize humans' mental activities in specific social circumstances along with their behavioral and affective responses \cite{meinhardt2018two,mehl2020theory}. 
% 每个chain里面包含五种基本要素，解释基本含义
Each cognitive chain involves five types of nodes: 
\textbf{1) \textit{situations}} denote the social circumstances;
\textbf{2) \textit{clues}} denote the trigger factors;
\textbf{3) \textit{thoughts}} denote the mental activities;
\textbf{4) \textit{actions}} denote the behavioral responses;
\textbf{5) \textit{emotions}} denote the affective responses.
Moreover, as shown in Figure \ref{fig-intro}, individuals react differently to the same situation due to the diversified cognitive processes of ToM. 
Therefore, for each situation, we derive multiple cognitive chains and further label them as \textbf{\textit{positive}} (means optimistic) or \textbf{\textit{negative}} (means pessimistic) to mark the chain polarity.
%Furthermore, people react differently to the same situation because they may have different cognitive processes. In the above example about \emph{delivering a talk}, one may positively think that \emph{he/she will deliver an impressive speech}, or in contrast, negatively think \emph{bad multimedia equipment hampers his/her performance}. Therefore, for the same situation, we derive multiple different cognitive chains to capture the diversity of ToM, and further label them as \texttt{Positive} or \texttt{Negative} to mark the chain polarity. 
We propose to induce the raw data from large language models, and then recruit educated workers majoring in psychology for manual selection and revision. The resulting knowledge graph constitutes 62,328 nodes and 45,369 cognitive chains.

The construction of \coke offers the basic ToM ability to understand and infer the human goals in already collected situations \cite{call2011tom30year}. But obviously, it is impossible to enumerate all situations in the real world. Thus we move one step further and build a cognitive generation model \cokelm to cope with unseen situations that have not appeared in the knowledge graph. Specifically, we decompose the construction of cognitive chains into four cognitive generation tasks, then finetune pre-trained language models (PLMs) using the manually collected data in \coke. By this means, we combine the commonsense knowledge embedded in PLMs and the ToM ability provided by \coke, enabling \cokelm to infer cognitive chains for unseen situations. %and make \cokelm capable of inferring the cognitive chains for unseen situations.

We summarize our contributions in this work as follows. \textbf{First}, we propose the first cognitive knowledge graph for machine theory of mind. We instantiate human theory of mind (ToM) as a collection of 45k$+$ manually verified cognitive chains, which provides a basic ToM ability for accessing and learning. \textbf{Second}, we build a powerful cognitive generation model \cokelm by associating \coke with pre-trained language models, so as to predict cognitive chains for out-of-KG situations. \textbf{Third}, we conduct extensive experiments to evaluate the ToM ability of \cokelm. The results show that \cokelm outperforms strong baseline models such as T5 \cite{RaffelSRLNMZLL20} and InstructGPT \cite{instructgpt} on both automatic and human evaluations in all cognitive generation tasks, which in turn demonstrates the high quality of \coke. \textbf{Fourth}, we further substantiate the potential of \coke in enhancing social applications. Upon the integration of \coke , there is a significant improvement in the performance of the Emotional Support Conversation (ESC) system \cite{DBLP:conf/acl/LiuZDSLYJH20}, validated by both automatic and human evaluation.
%A close look towards the generated cognitive chains further indicates that \cokelm effectively internalizes the ToM ability.




==> sections/02-related.tex <==

\section{Related Work}
\vspace{-0.5mm}
\subsection{Commonsense Knowledge Graph}
\vspace{-0.5mm}
Cognitive knowledge is essential for modeling intuitive tasks, such as reasoning, in language models.
% Add cite？
Previous work mainly focuses on realizing cognitive knowledge through commonsense.  
They construct text-based knowledge graphs that include numerous instances of Head-Relation-Tail triplets regarding different events and objects.
One of the widely-used examples of such knowledge graphs is ConceptNet \cite{Speer2016ConceptNet5A}, which provides a graph of concepts connected by relations, covering a variety of taxonomic facts. 
\citet{Sap2019ATOMICAA} proposed ATOMIC, a graph of if-then inferences that models social commonsense in daily life events. 
Similarly, CICERO \cite{ghosal-etal-2022-cicero} provides a dataset of dyadic conversations with 
%five types of 
reasoning-based commonsense inferences.
GLUCOSE \cite{mostafazadeh-etal-2020-glucose} focuses on implicit commonsense knowledge in narrative contexts.
% \cite{mostafazadeh-etal-2020-glucose} created GLUCOSE to model implicit commonsense knowledge in narrative contexts.
% However, by only modeling commonsense, previous work fails to capture the importance of situational context and cognitive processing of the individuals involved in an event, which is essential for realizing cognitive knowledge.

% Add our work...
The most relevant to our work is ATOMIC \cite{Sap2019ATOMICAA}, which considered event-centered commonsense relations, such as temporal relationships (e.g., \textit{IsBefore} and \textit{IsAfter}) and causal relationships (e.g., \textit{Causes} and \textit{xReason}).
But it is challenging for the above knowledge to enable AI systems to be cognitively inferring, and the cognitive process of human behavior is still under-explored.
% The cognitive process involves a wider range of dimensions, requiring the system to understand the user's situation, infer their inner thoughts, and predict the following behavior.
To alleviate this limitation and advance related research, we consider ToM and propose the first cognitive knowledge graph, \coke, aiming to enhance the cognitive inference capabilities of AI systems.
Compared with existing knowledge graphs, \coke considers more dimensions of cognitive reasoning and adopts the chain structure to build diverse cognitive processes.% under the same situation.

\subsection{Data Collection from LLMs}
With the recent advances in pre-trained large language models such as GPT-3 \cite{BrownMRSKDNSSAA20}, many researchers have begun to leverage such models to induce valuable data for various tasks. 
\citet{west2021symbolic} prompted GPT-3 to distill commonsense knowledge, while \citet{kim-etal-2022-soda} leveraged it to create a large-scale dataset of socially-grounded conversations. 
Similarly, \citet{wang2021towards}, \citet{yoo-etal-2021-gpt3mix-leveraging}, and \citet{augesc} used LLMs to augment training data for better performance.
%text classification, and
%Such models have also been used for data augmentation from current existing datasets \cite{yoo-etal-2021-gpt3mix-leveraging}.
%\citet{augesc} simulated emotional support conversations using GPT-J \cite{gptj} to augment the original dataset. 
% Therefore, we found it intuitive to leverage LLMs for our task.

Despite the powerful generative capabilities of language models, using them for knowledge graph construction involves more implicit knowledge and expressions than data augmentation for other tasks.
\citet{BosselutRSMCC19} showed that language models trained on knowledge graphs can effectively alleviate this problem, and the resulting inference models can augment effective commonsense knowledge triples.
In our work, we control the quality of the constructed \coke by carefully designing the prompt and combining the steps of model generation and manual annotation. We show that the cognitive generation model \cokelm obtained by fine-tuning on this data can generate valid cognitive chains as well. 









% \subsection{Comparison to Other Resources}
% To evaluate the originality of CKG Knowledge, we compared its characteristics to those of the two most pertinent knowledge graph resources: ConceptNet \cite{Speer2016ConceptNet5A} and ATOMIC \cite{Sap2019ATOMICAA}. ConceptNet represents commonsense knowledge as a graph of concepts connected by relations. Its knowledge consists of taxonomic facts such as "Tiger is an animal." Atomic focuses on general events and the associated social commonsense. The if-then inferences in nine dimensions allow it to cover the most causal relations for common sense inference. 
% CKG focuses on situational context and the cognitive processing of humans relating to them. It encompasses the majority of cognitive reasoning's causal relations. The structure of the graph clearly demonstrates the distinction between cognitive and commonsense reasoning. 
% Both ConceptNet and Atomic provide structures for point-to-point mapping. Therefore, the tail nodes inferred from the same head are parallel and unrelated. As a cognitive graph, cognitive reactions serve as the hinge between the external situations and the individual's reaction. In addition, the schema of information from various perspectives about circumstances influences cognitive response inference. This is why we utilize the chain structure.

% In addition to the structural difference, the defined relation type in our graph are more congruent with human cognitive processes, and the content offer more information cognitive processes.
% When presented with a particular scenario, a person will formulate a cognitive reaction based on all the relevant facts.
% In the event from Atomic, the cognitive situation cannot consist of generic short sentences with abstract person names such as PersonX and PersonY. Even in comparable settings, the diverse relationships between the second character and the subject (Family Relationship, Collegial Relationship, and Couple Relationship) might evoke distinct cognitive reactions from the subject.

==> sections/03-coke.tex <==
\section{\coke: Cognitive Knowledge Graph}
% \begin{figure*}[t]
% 	\centering
% 	\vspace{-6mm}
% 	\hspace{0mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	\includegraphics[width=0.98\linewidth]{figures/dimension}
% 	\centering
% 	\caption{An overview of five types of nodes and their definitions in \coke.}
% 	\label{fig-dimension}
% 	\vspace{-6mm}
% \end{figure*}
\subsection{Preliminaries}
\label{sec-tom}
\begin{comment}
% ToM 的定义 ： 理解他人的心理状态和情感， 从而理解和预测他人的行为反应
Theory of Mind (ToM) \cite{call2011tom30year} is the ability to understand other people's mental states and emotions and understand and predict their behavioral reactions.
% 理解情感 不仅依赖于 社交场景，还依赖于 人对于社交场景的认知反应（cognitive response === thouhgt (一种mental state)）
Understanding emotion depends not only on the objective features of the situation but also on the cognitive response that the situation brought to \cite{harris1989young}. 
% 预测他人的行为，依赖于心理状态。 心理状态会  因为场景中不同的社会线索  而有区别。
Predicting the behavior of others involves the mental state (intentions, beliefs, and thoughts).
These mental states are differentiated from observable social cues conveyed in different perspectives (like human action, motion, and personality) related to the social situation \cite{MeinhardtInjac2018TheTA}. 
% 由此可见，ToM inference 所涉及到的五个内容，相互关联 且形成链式结构。
Thus, it can be seen that the five concepts (social situation, social cues, mental state, affective and behavioral reaction) of the Theory of Mind inference are interconnected and formed in a chain structure.
\end{comment}
\paragraph{What is Theory of Mind?} Theory of Mind (ToM) refers to the ability of humans to understand and infer other people's desires, beliefs, and intentions \cite{premack1978tom}. The development of ToM begins very early in childhood, around 2 to 5 years old \cite{carlson2013theory}, and plays an important role in human social communication and relationship building \cite{giovagnoli2019theory}. 
Under specific social circumstances (\textbf{\textit{situations}}), the core mechanism by which ToM empowers us is to ascribe others' {mental activities} (\textbf{\textit{thoughts}}), and predict their corresponding {behavioral responses} (\textbf{\textit{actions}}) and {affective responses} (\textbf{\textit{emotions}}) \cite{leslie2004core,apperly2010mindreaders}. Furthermore, the acquisition of ToM enables us to realize and appreciate that people can have different cognitive responses in the same situation due to various {trigger factors} (\textbf{\textit{clues}}) like personality and experience \cite{meinhardt2018two}.

%\input{tables/dimension.tex}
\paragraph{Why Do AI Systems Need ToM?} 

% 为什么需要
% ToM 是AI system 一直追求的一种能力 （cite Sap2022NeuralTO）
% AI系统的发展目标是做出更贴合人的需求的操作。
% 他们追求理解人的处境的能力这种能力，从而更有效的操作。 (cite Langley2022TheoryOM)


Theory of Mind (ToM) has been a persistent yet elusive goal of artificial intelligence for decades \cite{choi2022curious}. AI systems need ToM to understand a user's situations and predict subsequent reactions, so as to provide effective responses or operations that meet the user's needs \cite{Le2019RevisitingTE,Dhelim2021IoTEnabledSR,Langley2022TheoryOM}. 
However, recent studies \cite{Sap2022NeuralTO} show that one of today's largest language models (GPT3) \cite{BrownMRSKDNSSAA20} still lacks ToM and social intelligence. The main reason is that AI systems can only learn from text corpus in training, but cannot access the human mental state and cognitive process that determine what and why to say. At present, there are neither public resources that contain all the concepts in ToM, nor commonsense knowledge graphs that depict the structure of cognitive chains in ToM. This motivates us to propose the first cognitive knowledge graph for the machine theory of mind.

%%%%%=====================================

%%%%%%   static data 需不需要 cite?
% 静态文本
    %特征： self-contained and written for general purpose 
% 系统问题：
    %无法 access to the communicative intent or to alternatives
    %意味着 系统无法 利用 文本之间 在 心智层面关系 
    
% The main reason is that the AI systems can only learn from self-contained static texts that written for a general purpose during training but cannot access the communicative intent or alternatives to use the inference between the texts at the Theory of Mind level.
% 








%%%%%=============================================
% 对于传统的AI system, ToM 能力的加入后： 
% 例如， 
% 语音助手的例子： （做了什么，解决了什么，达到了什么）( cite (Dhelim2021IoTEnabledSR))
% 站在别人的角度分析用户的下一步的行动   
% 做出了贴合人需求的响应， 
% 增强人与系统的互动和贴合人的需求  
%一个对话系统的例子： （做了什么，解决了什么，达到了什么） (cite(Le2019RevisitingTE)
% 站在别人的角度 分析所处的环境 分析人的心理状态。  （基于他人所处的环境对心理状态分析）
% 以对话历史的背景 对模糊的表述进行推理。
% 增加了系统与用户的交流

%For the technologies where AI is used to interact with users, e.g., voice assistants, higher-order ToM ability lets them give considerate system responses \cite{Dhelim2021IoTEnabledSR} based on the situation analysis and action prediction, such as giving travel advice if someone asks about the weather in a certain place.
%For the technologies where AI is used to adapt to users,e.g., AI-assisted counseling, ToM ability helps the dialogue system resolve ambiguous references\cite{Le2019RevisitingTE} by predicting the users' mental states based on the dialogue history so as enhance the communication between users and the system.


% 为什么没有
% 现有的工作没有很好的分解 Theory of Mind 的任务, 让语言模型去学习 Theory of Mind 
% 仅仅是利用 a false-belief task 去判断语言模型的 Theory of Mind 的能力 (cite(Grant2017HowCM))
% a false belief 测试的是: 回答和故事相关的问题 ,问题是和mental state 相关      
% 任务的分解问题：
% 数据中跟多是故事中人 Mental State 的推测 
% 不包含ToM 涉及的其他的反应的推测。
% 任务的设置形式问题：
% 任务的设置并不符合我们日常对于AI系统的运用 ： 问答

% 除去目前ToM有的单项选择任务的数据以外，没有很好的符合Theory of Mind 推理关系的结构的图谱和数据
% 没有图谱包含ToM 推理所需要的所有元素帮助LLM 学习 ToM
% 此外现有的图谱结构也并不符合ToM的推理流程。

%Theory of Mind inference needs to be decomposed into tasks well to let LLM  learn and use it in realistic scenarios.  \citet{Grant2017HowCM} proposed the False-Belief task to evaluate the capability of LLM to form the Theory of Mind. The task was cast as a question-answering task that gives a story and lets systems answer questions about only the mental states of agents in that story.  However, more concepts involved in the Theory of Mind inference, such as the affective and behavioral responses, should have been mentioned. Besides, the task form in the question-answering task is suitable for evaluating the LLM, but it takes more work for LLM to learn and utilize the ToM.
%Until now, no resource contains all concepts in the ToM inference and is in a suitable structure matching the flow of the ToM inference.

% 静态文本的问题
    % for general audience  不包括 文本背后的通用知识
    % 不包括语句背后的意图（intend or mental states）
    % 从主人公的角度 单一视觉的描述
% 因此 基于静态文本训练的模型无法
    % 无法利用个人世界的知识
    % 从不同人的角度。
    % 推测并利用他人的心理状态

% The static text written for the general audiences does not  offer universal knowledge and intent of the sentence. And it describes only one protagonist and his relation to his surroundings from a single point of view.
% So that the LLMs trained on these data cannot reason about the mental states of different characters in situations using self-world knowledge like people, which is highly predictive of the pragmatic inferences.





%\subsection{Graph Structure}

% \begin{figure*}[t]
% 	\centering
% 	\vspace{-6mm}
% 	\hspace{0mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	\includegraphics[width=0.98\linewidth]{figures/dimension}
% 	\centering
% 	\caption{An overview of five types of nodes and their definitions in \coke.}
% 	\label{fig-dimension}
% 	\vspace{-6mm}
% \end{figure*}

\begin{figure*}[h]
	\centering
	\vspace{0mm}
	\hspace{-10mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
	\includegraphics[width=0.80\linewidth]{figures/data_collection_cz}
        % \includegraphics{figures/data_collection.png}
	\centering
	\caption{The two-step data collection approach for constructing \coke.}
	\label{fig-datacollection}
	\vspace{-4mm}
\end{figure*}





\subsection{Data Structure of \coke}
% 先点、再链、再类别
%总： 我们用链式结构
%和别的图谱结构的不同的结构
%更符合 cognitive process

% 根据心理学对心智理论的研究，我们将知识图谱设置为连锁结构，以更好地匹配认知过程的流程。
According to the above-mentioned psychology research on theory of mind, we specify five types of nodes in \coke: \textit{\textbf{situations}}, \textit{\textbf{clues}}, \textit{\textbf{thoughts}}, \textit{\textbf{actions}}, and \textit{\textbf{emotions}}. In Figure \ref{fig-dimension}, we present a quick overview of the node definitions and example cognitive chains. We here define the basic unit of \coke as the following cognitive chain: \textit{Situation{$\Rightarrow$}Clue{$\Rightarrow$}Thought{$\Rightarrow$}(Action$+$Emotion)}. This structure depicts the intact cognitive process of ToM: When a person faces a situation, some clues trigger his/her thoughts, along with his/her actions and emotions. Furthermore, to distinguish whether a cognitive chain is optimistic or pessimistic under the specific situation, we further define its polarity as \textbf{\textit{positive}} or \textbf{\textit{negative}}. In practice, the polarity of the cognitive chain is determined by its thought node. Notice that, in \coke, we omit the definition of edges (i.e., the connections between nodes) since they can be easily inferred when the types of nodes are already known. 
We then illustrate the nodes in detail.

\begin{comment}
\begin{figure*}[h]
	\centering
	\vspace{0mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	\includegraphics[width=0.98\linewidth]{figures/dimension}
	\centering
	%\caption{An overview of five types of nodes and their definitions in \coke.}
	\caption{ \coke instantiates the Theory of Mind as cognitive chains in social situations containing five types of nodes.}

	\label{fig-dimension}
	\vspace{0mm}
\end{figure*}
\end{comment}
\begin{comment}
  %we set the knowledge graph to the chain structure to better match the flow of the cognitive process. 
% 现有的知识图谱
%Current Knowledge graphs provide structures for point-to-point mapping. Therefore, the tail nodes inferred from the same head are parallel and unrelated.
% 和现有的知识图谱不同，在认知推理的过程中，前一个推理的尾节点 会在后去的推理过程中运用。
%During the cognitive process, the tail nodes may work as a part of the head nodes in the cognitive chain.
% 例如 图谱重的想法节点 作为着理论中的cognitive response  连接了外界场景和个人反应
%For example, the thought dimension serves as the hinge between the external environment and the individual's reaction.
%从外部环境推断出的思维维度    作为头部节点的一部分发挥作用 并影响情感和行为反应的推断。
%The thought dimension inferred from the external environment work as a part of the head node and affect the affective and behavioral reaction inference
% 因此 链式结构的知识图谱更符合认知流程从而帮助语言模型学习ToM 能力
%This is why we utilize the chain structure, which is more aline with the cognitive process and improves the ToM of the language models.

% 每一个场景有两类链式，正向链式和负向链式。 链式的极性 anchor 在cognitive reponse 中


%总
% 我们对cognitive chain 定义了4个dimensions  
% 对于同一个场景，我们定义正负两种链式结构。


% 定义dimension也是我们的contribution，方便 annotator筛选数据
% 我们定义了四类dimension，分别是：
%One of our contributions is to define five nodes for the cognitive chain in the Theory of Mind inference, which lets the lay annotators collect high-quality knowledge from raw data. 
%Based on the psychology research on the Theory of Mind, the dimensions comprise the pertinent \emph{clues} associated with the social situation, social situation-related \emph{thought} in dual polarity, and the \emph{action} and \emph{emotion} navigated by the thought. 



% 对于同一个场景，我们定义正负两种链式结构。
% 链条的极性 取决于 thought 
% 原因： 即使是陷入糟糕的场景，积极的想法也会带来积极的情感
%For one social situation, we define two kinds of cognitive chains: negative cognitive chain and positive cognitive chain. 
%Whether the chain is positive or negative is anchored to the thought.
%Since even people get into a bad situation, positive thoughts let them have positive emotions.

%Following, we give detailed definitions of dimensions.  
\end{comment}


%Situation 的定义和覆盖内容
\textbf{{\emojisituation} Situations} in \coke denote the social circumstances in which individuals (potentially) interact with others. By referring to DailyDialog \cite{LiSSLCN17}, a widely used daily social dialogue dataset, we select the five most common social topics: \textit{School} (what happened at school), \textit{Work} (what happened at work), \textit{Tourism} (travel and entertainment), \textit{Relationship} (social activities between individuals), \textit{Ordinary Life} (what happened in families). Detailed information about each topic can be found in the supplementary \textit{Technical Appendix}.


% Detailed information about each topic can be found in Appendix \ref{appendix-topicinfo}.
% The details of processed features can be found in the supplementary \texttt{Technical Appendix}.




% 数据收集的流程图
% 图片描述：
%1. 图片中描述了五个concept的收集顺序。
%2. 每个concept收集分为三步， 分别是 设计prompt，PLM生成， quality control
%3. 对于每一个prompt，设计了 3个example，具体细节可以在appendix中看到
%4. 根据第一行的任务描述 我们让PLM生成初始数据
%5. 我们对PLM生成任务进行自动化筛选 和人工筛选修改 得到最终的知识图谱。

% Clue 定义和类别
% Clue 的定义
    % 当我们进入一个场景中，我们会观察到  场景中的细节信息   和   回溯我们已知的场景相关知识。 cite(Dumova2009HandbookOR)
    % 我们decode 这些message 做出认知回应  cognitive response 
    % 我们定义这些message 为场景相关的线索
    % 这些场景相关的线索 使我们对 同一个场景的产生不同的想法 （具体化和差异化想法）
% Clue 的分类
    % 我们将Clue 进行了归类。
\textbf{{\emojiclue}Clues} in \coke denote the trigger factors that direct and concretize the cognitive process. In a specific situation, humans' mental activities are triggered and directed by relevant subjective and objective factors \cite{meinhardt2018two}. According to the taxonomy from \cite{baldwin1992relational}, clues mainly involve the particular information about personality, knowledge, experience, education, objective facts, social rules, and so on.


%When we participate in a situation, we observe the detailed information related to the situation  and retrace our knowledge to the situation.
%Once we decode these messages, we give our thoughts to the situation.
%We define these messages as clues. 
% 我们没有直接标注 clue 的类别。
% 但是我们考虑了以下的四类定义的 clue 
%The different clues to the situation concretize and differentiate our thoughts \cite{baldwin1992relational}.	
%We divide these clues into four categories: 
\begin{comment}
\begin{itemize}
	\item[$\bullet$]Other Clue: particular information about the others’ appearance, actions, personality, etc.
	\item[$\bullet$]Person Clue: particular information about our appearance, actions, personality, etc.
	\item[$\bullet$]Object Clue: how people comprehend what various items are, how they should work, and what to expect
	\item[$\bullet$]Social Clue: particular information about how people behave in social situations.
\end{itemize}
\end{comment}


% Thought 定义和类别
 \textbf{{\emojithought}Thoughts} in \coke denote the mental activities that act as the cognitive responses to situations. Thoughts serve as the bridge between the external environment and individual cognition, thus can be considered as the core of ToM \cite{Westbrook2007AnIT}. 
As mentioned before, the polarity of a cognitive chain is anchored to its thought node. In other words, an optimistic thought marks the entire cognitive chain as positive, and a pessimistic thought marks it as negative.

 \textbf{{\emojiaction}Actions} in \coke denote the behavioral responses to situations after specific thoughts. Notice that the semantic meaning of actions may not conform to their polarity annotations. For example, in Figure \ref{fig-dimension}, the action ``\textit{I practice my script in front of the mirror}'' is a neutral sentence. However, it is actually the consequence of the negative thought ``\textit{I may mess up the speech}'', so it is still labeled as negative.

%As shown in Figure\ref{fig-intro}, if someone believes that \emph{"he will give an impressive speech"}$_{Thought}$, he may \emph{"have a restful sleep tonight"} $_{Action}$. Or he may \emph{"practice in front of the mirror" }$_{Action}$ to avoid \emph{"messing up the talk"} $_{Thought}$.
%Under the situational context, more cognitive information is engaged in cognitive processing, leading to the inference of actions that are more specific and consistent.


% Emotion 定义和类别
\textbf{{\emojiemotion}Emotions} in \coke denote the affective responses to situations after specific thoughts. Without loss of generality, we restrict the emotions to six basic categories \cite{shaver1987emotion}: \textit{Love}, \textit{Surprise}, \textit{Joyful}, \textit{Sad}, \textit{Angry}, and \textit{Fearful}. The first three appear in positive cognitive chains, while the last three appear in negative cognitive chains.

%We assign an emotion label to describe someone's feeling evoked by a specific thought in a social situation. 
%When we utilize the Pre-trained Language Model to generate emotion labels automatically, more than a hundred emotional words are generated to describe the feelings, which is hard to annotate manually. We classify them as positive and negative and label them with six basic emotions (Love, Surprise, Joyful, Sad, Angry and, Fearful).







% \begin{figure*}[h]
% 	\centering
% 	\vspace{-10mm}
% 	\hspace{-10mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
% 	\includegraphics[width=0.85\linewidth]{figures/data_collection_cz}
%         % \includegraphics{figures/data_collection.png}
% 	\centering
% 	\caption{The two-step data collection approach for constructing \coke.}
% 	\label{fig-datacollection}
% 	\vspace{-4mm}
% \end{figure*}

\subsection{Data Creation and Selection}
Recent studies have proved that large language models (LLMs) trained on huge text corpora can naturally serve as a repository for data collection \cite{MehriAE22,kim2022soda}. 
% collection \cite{MehriAE22, kim-etal-2022-soda}.
Inspired by their successful attempts, we propose a two-step data collection approach for constructing \coke. As shown in Figure \ref{fig-datacollection}, \textbf{1)} we first manually design suitable few-shot prompts to induce InstructGPT
%\footnote{We use {\texttt{text-davinci-002}} offered by OpenAI API.} 
\cite{instructgpt}  to automatically generate raw data for five types of nodes in a pipeline manner. \textbf{2)} We then recruit and train eight graduate students majoring in social psychology as annotators to select and revise the outputs of InstructGPT. Next, we illustrate the details of how to prompt InstructGPT, then introduce the data statistics after human annotation. For clarity, more detailed parameters and templates used for prompting are provided in the supplementary \textit{Technical Appendix}.

% Inspired by their successful attempts, we propose a two-step data collection approach for constructing \coke. As shown in Figure \ref{fig-datacollection}, \textbf{1)} we first manually design suitable few-shot prompts to induce InstructGPT\footnote{We use \href{https://beta.openai.com/docs/model-index-for-researchers}{\texttt{text-davinci-002}} offered by OpenAI API.} \cite{instructgpt}  to automatically generate raw data for five types of nodes in a pipeline manner. \textbf{2)} We then recruit and train eight graduate students majoring in social psychology as annotators to select and revise the outputs of InstructGPT. Next, we illustrate the details of how to prompt InstructGPT, then introduce the data statistics after human annotation. For clarity, more detailed parameters and templates used for prompting are provided in the supplementary \textit{Technical Appendix}.



\begin{comment}
    % 我们利用了 语言模型 并 人工筛选了数据
% 
%我们利用预先训练好的语言模型IntructGPT来生成每个维度的原始数据，并手动选择和修改它们以获得有用的数据。
%为了确保我们的知识图谱的高质量，我们检测并选择了八个社会心理学研究生作为注释者。
%我们给他们每个维度的详细定义和关于注释的详细指导。
%对于每个维度的构建，我们有三个步骤： \ref{fig-datacollection}
    %1. 设计提示中的例子；
    %2. 把我们选择的输入给PLM；
    %3.自动选择数据和手动选择并修改数据
% 在下文中，我们将展示我们如何从模型中获得原始数据，以及如何训练注释者为每个维度填写不合理的数据。
%We utilize the pre-trained language model InstructGPT to generate the raw data for each dimension and manually select and revise them to get useful data. To ensure the high quality of our knowledge graph, we detected and chose eight social psychology postgraduate students as annotators. We give them detailed definitions of each dimension and detailed guidance about the annotation. 
%As shown in the Figure \ref{fig-datacollection}, for each dimension construction, we have three steps:\textcircled{1}  design the examples in the prompt \textcircled{2} give the PLM the selected input we want to make inference on  \textcircled{3} automatically select data and manually select and revise data
%In the following, we demonstrate how to obtain raw data from the model and how we train the annotators to retain reasonable inferences for each dimension.
\end{comment}
\begin{figure*}[h]
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{1mm}

% \vspace{2mm}
\vspace{0mm}

\subfigure[]{
\hspace{-2mm}
\includegraphics[width=0.32\textwidth]{figures/data_situation_col3}
\label{fig-data_situation_col3}
\hspace{-2mm}
\vspace{0mm}
}
\subfigure[]{
\includegraphics[width=0.32\textwidth]{figures/data_posthought_col3}
\label{fig-data_posthought_col3}
\hspace{-2mm}
\vspace{0mm}
}
\subfigure[]{
\includegraphics[width=0.32\textwidth]{figures/data_negthought_col3}
\label{fig-data_negthought_col3}
\hspace{-2mm}
\vspace{-2mm}
}

\centering
\caption{Prompting LLMs for (a) situations, (b) positive thoughts, and (c) negative thoughts.}
\label{fig-data-thought}
\vspace{-5mm}
\end{figure*}

% Situation 的定义和内容
% 我们找不到合适的数据集
    % 现有数据集的问题
% 如何利用 GPT生成 Situation

% 我们的认知知识图谱包含了各种各样的日常社会情况。它以第一人称叙述的方式描述了我们日常生活中的社会环境。
%我们需要： 
    % 1. 我们需要有内容且覆盖日常生活的场景
    % 2. 且场景中人物之间的关系明确。
%但是我们无法在现有的数据库中找到大量的数据。
\paragraph{Prompting LLMs for {\emojisituation}Situations}
{{Situations}} in \coke denote the social circumstances in which individuals (potentially) interact with others, which exhibit a strong correlation with social events and describe the social environment of daily lives. Unfortunately, to the best of our knowledge, there is no public dataset that contains a wide variety of social situations. Therefore, we choose the events in ATOMIC \cite{Sap2019ATOMICAA}, a frequently-used commonsense knowledge graph for if-then reasoning, as an alternative. However, the events from ATOMIC are still not qualified to become the situations in \coke. The reasons are two-fold, and we here take the event ``\textit{PersonX misses calls from PersonY}'' as an example. \textbf{1)} ATOMIC events replace the characters with ``\textit{PersonX}'' and ``\textit{PersonY}'', thus having lost most of the interpersonal information that is indispensable for social situations. For example, if someone misses calls from his employer, he may worry that something is wrong with his work. But if the caller changes to his girlfriend, he may sense love because she cares about him. \textbf{2)} ATOMIC events omit most of the social context information, making the background environments where the events occur not available. For example, we don't know if the calls in the above event happen at work or on vacation, so we have no idea how to reify subsequent cognitive processes.

% \begin{figure}[h]
% 	\centering
% 	\vspace{-1mm}
% 	\hspace{0mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
% 	\includegraphics[width=0.42\textwidth]{figures/data_situation_cz}
%         % \includegraphics{figures/data_collection.png}
% 	\centering
% 	\caption{Prompting LLMs for situations.}
% 	\label{fig-data-situation}
% 	\vspace{-2mm}
% \end{figure}

To address the above problem, we choose to prompt InstructGPT, one of the most powerful LLMs, to rewrite ATOMIC events to qualified \coke situations. Specifically, we first manually create several demonstration (input, output) pairs such as (``\textit{PersonX misses calls from PersonY}'', ``\textit{I miss multiple calls from my girlfriend because I’m playing Project Zomboid}''). Then we wrap the demonstrations with the task instruction (``\textit{Translate [Event] to [Situation]}'') and an arbitrary event query (``\textit{PersonX delivers PersonX's message}'') to form an input template as shown in Figure \ref{fig-data_situation_col3}. 
% Figure \ref{fig-data-situation}. 
As a result, we collect the output situation from InstructGPT like ``\textit{I will deliver a talk at the university tomorrow}''. 
% More detailed parameters and templates used for prompting can be found in the supplementary \textit{Technical Appendix}.
% For clarity, we omit the detailed parameters and templates used for prompting. More information can be found in Appendices \ref{appendix-gpt3para} and \ref{appendix-gpt3prompt}. 
In practice, we manually select 400 ATOMIC events that are general and easy to adapt, then rewrite each event to 5 situations with different topics. Finally, we obtain \textbf{2,000} raw situations.
%Our cognitive knowledge graph encompasses a wide variety of social situations, which describes the social environment of our daily lives in first-person narrative. 
%These contextual situations describe the base event with detailed character relationships.

%最相关的知识图谱Atomic给出了事件短语作为基础事件。他们用'PersonX'和'Person Y'代替主语和其他角色，只留下包含动词谓语和其参数的动词短语。
%然而，我们的认知反应受到我们与情境中其他角色或潜在角色的关系的影响。
%例如，如果我错过了雇主的多个电话，我就会担心我的工作出了问题。如果我错过了我女朋友的几个电话，我就会感觉到她对我的思念之情。
% （图1 没有很合适的例子 证明这一点，给了一个新的例子）
%We cannot find a large number of data in the available databases as situations in our graph. 
%The most relevant knowledge graph Atomic gives event phrases as the base events. They replace the subject and other characters with 'PersonX' and 'Person Y', leaving just verb phrases containing a verb predicate and its arguments. However, our cognitive chain is influenced by our relationships with the other characters or potential characters in the situations. For example, if I miss multiple calls from my employer, I will worry that something is wrong with my work. If I miss several calls from my girlfriend, I sense the love that she misses me. \\

% 我们花了很多时间生成和筛选 social situation
% 为了保证 话题的丰富和多样性，我们筛选并扩展了Atomic 基础事件到 situation
% 首先 我们需要筛选出适合扩展的基础event.
    % Atomic Event 涉及4类关系，分别是 PersonX, PersonX and PersonX's, PersonX and PersonY, and PersonX and PersonY's.
    % 我们将整个Atomic 根据关系分为四组。
    % 每一组中包含同一个动词的事件我们只随机保留 1 个
    % 我们删掉含有不安全关键词的事件。
    % 在每组中选择50个event 得到400 个基础event。
% 我们需要设计 PLM的prompt内容。
    % 我们为5个topic,每一个topic 准备了 一个prompt Example。 为了使话题均衡
    % Example中包含四类关系和对应的扩展situation             ref(Situation 生成图)
    % 我们将筛选出的基础事件 和 每一个Example 组成combo 给语言模型。 最终得到2000个situation
    % 删除掉相近的场景确保场景的多样性。 并确保话题的均衡。 我们选择了1200个situation
    
%Therefore, we devote much effort to creating and selecting social situations. 
%为了保证 话题的丰富和多样性，我们筛选并扩展了Atomic 基础事件到 situation
%In order to ensure broad and diverse coverage, we expand the base event with different relationships and rich social content to social situations, covering five common daily topics. 
%Firstly, we need to select base events that are suitable to be extended. 
% 首先 我们需要筛选出适合扩展的基础event.
%We divide the Atomic data into four groups with distinct relationships: PersonX, PersonX and PersonX's, PersonX and PersonY, and PersonX and PersonY's. 
%We retain one base event per verb in each group.  
%We deleted the base events that contained unsafe words.
%We finally selected 400 base events that are more general and easy to be extended.

% 我们需要设计 PLM的prompt内容。
% 为了使得话题均衡，我们为每个话题设计了一个prompt examples template
% 每一个 prompt template 包含四类关系的四个examples
% 我们将任务描述，prompt template 和 新的基础事件 输入给语言模型
%Moreover, we designed a prompt example for each topic to let PLM generate situations averaged in topics. four base events in four relationships and their accompanying social situation examples are condensed into a prompt example. 
%The selected new base events combined with each prompt template are given PLM and lead the few-shot generation. 
%We have screened all situations with various character relationships and social content to retain situations with high content variability from all situations.
%Finally, we get 1200 situations.

% \begin{figure*}[h]
% \setlength{\abovecaptionskip}{1mm}
% \setlength{\belowcaptionskip}{1mm}

% \vspace{2mm}
% \subfigure[]{
% \hspace{-2mm}
% \includegraphics[width=0.32\textwidth]{figures/data_situation_col3}
% \label{fig-data_situation_col3}
% \hspace{-2mm}
% \vspace{0mm}
% }
% \subfigure[]{
% \includegraphics[width=0.32\textwidth]{figures/data_posthought_col3}
% \label{fig-data_posthought_col3}
% \hspace{-2mm}
% \vspace{0mm}
% }
% \subfigure[]{
% \includegraphics[width=0.32\textwidth]{figures/data_negthought_col3}
% \label{fig-data_negthought_col3}
% \hspace{-2mm}
% \vspace{0mm}
% }

% \centering
% \caption{Prompting LLMs for (a) situations ,(b) positive thoughts, and (c) negative thoughts.}
% \label{fig-data-thought}
% \vspace{-5mm}
% \end{figure*}


\paragraph{Prompting LLMs for {\emojithought}Thoughts} Thoughts in \coke denote the mental activities that act as the cognitive responses to situations. As mentioned above, thoughts serve as the bridge between the external environment and individual cognition, and can be seen as the core of ToM. Since thoughts are triggered by certain clues, they come after clues in cognition chains. However, our pilot experiments show that directly using situations to prompt LLMs can better stimulate their generation ability and get more diverse thoughts, which is beneficial to manual selection and revision. Therefore, here we temporarily reverse the order of thoughts and clues, i.e., we first prompt LLMs using situations to generate thoughts, and then prompt LLMs using thoughts to generate clues.

% \begin{figure}[h]
% 	% \centering
% 	% \vspace{2mm}
% 	% \hspace{0mm}
% 	% \setlength{\abovecaptionskip}{1mm}
% 	% \setlength{\belowcaptionskip}{1mm}
% 	% \includegraphics[width=0.48\textwidth]{figures/data_thought_cz}

%   % \includegraphics[width=0.48\textwidth]{figures/data_thought_cz_positive}
%   % \hspace{1in}
%   % \includegraphics[width=0.48\textwidth]{figures/data_thought_cz_negative}
	
%         \vspace{-10mm}
%         \subfigure[]{\includegraphics[width=0.5\textwidth]{figures/data_thought_cz_positive}}
%         \subfigure[]{\includegraphics[width=0.5\textwidth]{figures/data_thought_cz_negative}}

%         \centering
% 	\caption{Prompting LLMs for positive thoughts (a) and negative thoughts (b).}
% 	\label{fig-data-thought}
% 	\vspace{-4mm}
% \end{figure}


% \begin{figure}[h]
% 	\centering
% 	% \vspace{4mm}
%         \vspace{-4mm}
% 	\hspace{0mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	\includegraphics[width=0.42\textwidth]{figures/data_thought_cz}
% 	\centering
% 	\caption{Prompting LLMs for positive thoughts (top) and negative thoughts (bottom).}
% 	\label{fig-data-thought}
% 	\vspace{-4mm}
% \end{figure}

As shown in Figure \ref{fig-data_posthought_col3} and \ref{fig-data_negthought_col3}, 
we manually construct the demonstration as ``\textit{When [Situation], I feel great/terrible since I think [Thought]}'' and again wrap it with the task instruction and an arbitrary situation query to form the input template. Notice that we use different sentiment terms (``\textit{great}'' and ``\textit{terrible}'') to control the polarity (\textit{positive} and \textit{negative}) of the generated thoughts. Since the polarity of a cognitive chain is anchored to its thought, we have also controlled the polarity of the entire cognitive chain that will be generated. 
% The detailed parameters and templates for prompting are present in Appendices \ref{appendix-gpt3para} and \ref{appendix-gpt3prompt}. 
% The detailed parameters and templates for prompting are present in the supplementary \textit{Technical Appendix}.
After prompting, we obtain \textbf{14,400} raw thoughts, half of which are positive and the other half are negative.
%containing \textbf{7,200} positive thoughts and \textbf{7,200} negative thoughts.

% 生成的Thought是什么
% 我们如何利用GPT3 
%     输入GPT3的内容 
%     得到的结果有什么问题
% 我们做了什么样的筛选 



% 在人的认知处理工程中，人主动联想场景相关线索。分析线索得到想法。
% 不同的是， 我们在收集线索和想法的数据时， 我们先得到场景中我们所有可能出现的想法，再找到和场景相关造成这些想法的线索。
% 我们获取统一个场景下的正向和负向的想法

%In cognitive processing, people spontaneously observe and retrace the relevant clues of the situation. They get thoughts after decoding these clues.
%Differently, when we collect the data, we get all likely thoughts in the situations first and find the clues that differentiate these thoughts.
%We get the dual-polarity thoughts in each situation.


% 我们利用了 PLM 生成 Thought。
    % 首先我们设计了正向和负向两种 prompt. 
    % 在正向的prompt中 ，我们给了 3 个example
    % 每个Exampl中 用自然语言描述了 我们在一个场景中拥有的一个正向想法。
    % 我们将prompt example 和 自然语言描述的新的situation 给PLM
    % 以完成句子的形式，得到想法的原始数据
% ========== 正向和负向模版 内容有区别
%We design negative and positive prompt examples, respectively.
%In each prompt example, we give three samples.
%In each sample, we describe how we think in the given situation in natural language.
%PLM decodes the prompt example and description of a new situation and generates three candidate thoughts data by completing the sentence.

% 原始的想法数据有很多的问题
    % PLM 会生成相似的句子
    % 想法的极性是错误的
    % 想法不符合场景事实
    % PLM 容易生成除了想法内容以外融于的文本
% 因此，我们删除了相似和错误的句子，并修改保留了部分数据

%PLM is likely to generate the same sentences to the given input and generate content irrelevant to the task. 
%Besides, some candidate thoughts are in the wrong polarity and even conflict with the situation.
%We filter out the same or incorrect thoughts and revise the data to retain more thought data.
\begin{comment}
\begin{figure}[h]
	\centering
	\vspace{0mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
	\includegraphics[width=0.48\textwidth]{figures/data_thought_cz}
        % \includegraphics{figures/data_collection.png}
	\centering
	\caption{Prompting LLMs for thoughts.}
	\label{fig-data-thought}
	\vspace{-5mm}
\end{figure}
\end{comment}





% We automatically generate dual-polarity thoughts to the given situation by using the PLM. 
% With the few examples of the thoughts responses to the situations, we prompt the PLM to generate likely thoughts to the given situations. 
% The examples in different topics in the prompts show the PLM how people cognitively react to various situations and let it generate relevant thought by completing the sentence.

% An example of the final prompt for negative thought generation is "Complete the sentence: \\n When I will give a presentation at college, I feel terrible since I think I will freeze on stage. \\n When I was waiting in the waiting room for my last job interview, I felt terrible since I thought I would not be selected. \\n When my friend wanted to move into the house that I had up for sale, I felt terrible since I thought she might not leave when I wanted her to. \\n When my younger sister is getting married before I am, I feel terrible since I think"\\
% Eight social psychology graduate students working as annotators filter the pertinent thoughts. Starting with an initial set of about 15 thousand thoughts distilled from InstructGPT, we: filter out thoughts with the same content, conflict with the situations, and are in the wrong emotion.

\paragraph{{Prompting LLMs for {\emojiclue}Clues, {\emojiaction}Actions, and \emojiemotion}Emotions}
Clues in \coke denote the trigger factors that direct and concretize the cognitive process. Thus we construct the demonstrations as ``\textit{When [Situation], I think [Thought] since [Clue]}'' to prompt LLMs for clues. Actions and emotions in \coke denote the behavioral and affective responses to situations after specific thoughts. We hence construct the demonstrations as ``\textit{When [Situation], I think [Thought] so [Action]}'' and ``\textit{When [Situation], I think [Thought] and I feel [Emotion]}'' to prompt LLMs for actions and emotions. Since emotion belongs to predefined categories, we further modify its corresponding prompt to the question-answering form. 
% Due to space limitation, we put the details about prompting clues, actions, and emotions in the supplementary \textit{Technical Appendix}. 
After prompting, we finally obtain \textbf{29,364} raw clues, \textbf{29,364} raw actions, and \textbf{14,400} raw emotions. Notice that their polarities are already determined by previously generated thoughts.
% Due to space limitation, we put the details about prompting clues, actions, and emotions in Appendices \ref{appendix-gpt3para} and \ref{appendix-gpt3prompt}. 




\begin{comment}
\paragraph{{\emojiclue}Prompting LLMs for Clues}
% 生成的Clues 是什么
% 我们如何利用GPT3 
%     输入GPT3的内容 
% 我们做了什么样的筛选 
    %得到的结果有什么问题


% 和我们之前说的，我们先筛选出想法再得到和trigger 想法的clue.
As we illustrated before, we select the thought candidates first and find the clues that trigger these thoughts.
% 我们给 situation 作为background和可能的thought
During the data collection, given the situation as a background and the specific thought, the PLM supplies clues consistent with the background and triggers the specific thought. 
% 原始数据的问题：
    % 不能连接场景和想法的 clue: 
        %和situatio内容无关矛盾
        % 不能引发thought
    % 相似内容

In addition to being repetitious, many clues cannot connect the situation and people's thinking.
They are conflictive or irrelevant to the situation or cannot trigger thoughts. All of these phrases with incorrect patterns are filtered away.

\begin{figure}[h]
	\centering
	\vspace{0mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
	\includegraphics[width=0.48\textwidth]{figures/data_clue_cz}
        % \includegraphics{figures/data_collection.png}
	\centering
	\caption{Prompting LLMs for clues.}
	\label{fig-data-clue}
	\vspace{-5mm}
\end{figure}



\paragraph{{\emojiaction}Prompting LLMs for Actions}
% 输入的Action 是什么：对于同一个场景下的正负思维，人会采取不同的行为。 
% PLM的输入：    因此我们设定了两种hardprompt 给intructgpt.在每一种hard prompt中，我们给定四个不同的场景相关的clue和同一种极性对应的想法。
% PLM的输出： 让InstructGPT以完成句子的方式，对给定的场景和想法生成3个行为inference.
% 得到的结果有什么问题: 1. InstructGPT 会对同一个输入得到语义相似的多个输出。 2.行为和给的输入产生矛盾
% 我们做了什么筛选： InstructGPT 会对同一个输入得到语义相似的多个输出，我们筛选掉这些相似的数据。同时我们筛选掉和输入产生矛盾的行为预测。最终我们从原始数据中保留了约百分之67%数据作为。

People take different actions in the same situation based on negative or positive thoughts. Therefore, we develop two distinct types of prompts for PLM. In the negative hard prompt, we provide four situations with the related negative thought. In the positive hard prompt, we provide four situations accompanied by positive thoughts.
We provide InstructGPT with the prompt, one situation, and a corresponding thought, and it returns three likely actions by completing the sentence. PLM typically produces identical outputs. And certain candidate acts contradict the situation. We compare these raw data and retain around 68\%.

\begin{figure}[h]
	\centering
	\vspace{0mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
	\includegraphics[width=0.48\textwidth]{figures/data_action_cz}
        % \includegraphics{figures/data_collection.png}
	\centering
	\caption{Prompting LLMs for actions.}
	\label{fig-data-action}
	\vspace{-5mm}
\end{figure}
 





\paragraph{{\emojiemotion}Prompting LLMs for Emotions}
% 怎么用GPT3 
% 数据问题


% 怎么用的GPT3
    % 定义为多选任务
    % 对两个极性分别设计了Prompt Example
    % 每个一个sample里有三个例子覆盖了同一个极性下的三种情感标签
We define emotion generation as a multiple-choice task to let InstructGPT choose the emotion label to describe the feeling brought by the thought. 
For two classes of emotion labels, we give separate prompt examples.
Each example gives three samples covering three emotion labels in one class.
\begin{figure}[h]
	\centering
	\vspace{0mm}
	\hspace{0mm}
	\setlength{\abovecaptionskip}{1mm}
	\setlength{\belowcaptionskip}{1mm}
	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
	\includegraphics[width=0.48\textwidth]{figures/data_emotion_cz}
        % \includegraphics{figures/data_collection.png}
	\centering
	\caption{Prompting LLMs for emotions.}
	\label{fig-data-emotion}
	\vspace{-5mm}
\end{figure}


% 数据问题
    % 筛选掉了  不相关不正确的文本
    % 给出正确标签
However, GPT3 can automate redundant words so that many irrelevant statements are given to the question.
The annotators go through all data, remove these irrelevant or incorrect contents and give the correct emotional labels. 
\end{comment}


\paragraph{Human Selection and Revision}
After collecting the raw data, we manually annotate a small amount of data and formulate several rules to distinguish good data from bad data. Subsequently, we use the detailed definition of nodes in \coke and the filtering rules as a tutorial to train the eight annotators. After passing an annotation qualification test, they are asked to select and revise the raw data of five types of nodes. 
More details about human annotation can be found in the supplementary \textit{Technical Appendix}.
% More details about human annotation can be found in Appendix \ref{appendix-humanannotation}. 

\begin{comment}
As shown in Table \ref{tab-statistics}, the final reserved data contains 1,200 situations, 9,788 thoughts, 21,677 clues, 19,875 actions, and 9,788 emotions, resulting in an overall retention rate of around 70\%. This statistic proves that ToM ability exhibited by most powerful LLMs like InstructGPT is still not satisfactory enough even with delicate prompting, thus further emphasizing the necessity of our construction of \coke. After linking and ordering the obtained nodes, we instantiate ToM with a total of 45,369 cognitive chains in \coke, containing 23,252 positive chains and 22,117 negative chains in English. Example \coke data can be found in Appendix \ref{appendix-dataexample}.
\input{tables/data_statistic.tex}
\end{comment}
The final reserved data contains \textbf{1,200} situations, \textbf{9,788} thoughts, \textbf{21,677} clues, \textbf{19,875} actions, and \textbf{9,788} emotions, resulting in an overall retention rate of around 70\%. This statistic proves that ToM ability exhibited by most powerful LLMs like InstructGPT is still not satisfactory enough even with delicate prompting, thus further emphasizing the necessity of our construction of \coke. After linking and ordering the obtained nodes, we instantiate ToM with a total of \textbf{45,369} cognitive chains in \coke, containing \textbf{23,252} positive chains and \textbf{22,117} negative chains in English. Detailed statistics and sample data of \coke can be found in the supplementary \textit{Technical Appendix} and \textit{Code \& Data Appendix}.
% Detailed statistics and sample data of \coke can be found in Appendix \ref{appendix-dataexample}. 
%More data can be found in the \textit{Code \& Data Appendix}.

% \href{https://drive.google.com/drive/folders/144zK_KCsy4eFyMhRggL20zYCrWQOimjz?usp=drive_link}{here}.



% 数据信息
% 人工过程

% 作为第一个认知图谱
    % 链条数  45k
    % 节点数  65k 
    % 节点类别 5
    % 话题类别 5 
    % 场景个数 1200
    % 总节点数 89248
    % 总保留数 62329
%As the first cognitive knowledge graph, we present about 45k cognitive chains involved in five types of nodes: Situation, Clue, Thought, Action, and Emotion. Our knowledge graph consists of around 65k nodes based on 1200 social situations across five topics.



% 人工过程
    % 获取足够多的clue 对同一个situation 有多个thought 生成
    % 筛查所有数据保留部分数据
%Table \ref{tab-statistics} shows that we collect as many clues as possible for each situation.
%Therefore,  we can utilize these clues to draw diverse thought inferences about the same situation.
%In contrast to denotational tasks, in which experts select just one label as right, our annotators examine raw data (about 90k inferences) and retain about 65k reasonable inferences.




==> sections/04-cokelm.tex <==
\section{Cognitive Generation Model \cokelm}

\input{tables/cokelm_flow.tex}
%\textcolor{red}{Need a big figure to show the training process of \cokelm.}
% COKE提供了基本的ToM能力
By consulting the constructed cognitive knowledge graph \coke, we can obtain the basic ability of theory of mind (ToM) via matching the faced situation to a similar situation in KG, and then inspecting the involved cognitive chains (a.k.a, entity linking). But obviously, \coke only collects finite situations and cannot cover the infinite and diverse situations in the real world. Inspired by the methods for automatic knowledge graph completion like COMET \cite{BosselutRSMCC19}, we propose a cognitive generation model \cokelm to cope with unseen situations and expand the scope of application of \coke. \cokelm is built upon pre-trained language models (PLMs), aiming to integrate the commonsense knowledge inside PLMs and the ToM ability from \coke. To this end, we first decompose the cognitive process into a sequence of cognitive generation tasks, and then finetune the T5 model \cite{RaffelSRLNMZLL20} using the collected data from \coke. Next, we illustrate the details.


\subsection{Cognitive Generation Tasks}

In \coke, a cognitive process towards theory of mind (ToM) is instantiated as a sequenced cognitive chain containing situation, clue, thought, action, and emotion. Therefore, given a situation, we can decompose the cognitive process into four generation tasks as shown in Table \ref{tab-cokelm}. These four tasks work in a pipeline manner, and the complete cognitive chain can be restored by linking their generated results.

% In \coke, a cognitive process towards theory of mind (ToM) is instantiated as a sequenced cognitive chain containing situation, clue, thought, action, and emotion. Therefore, given a situation, we can decompose the cognitive process into  four generation tasks: \textbf{Clue Generation}, \textbf{Thought Generation}, \textbf{Action Generation} and \textbf{Emotion Generation}. These four tasks work in a pipeline manner, and the complete cognitive chain can be restored by linking their generated results.

\textbf{Clue Generation}. 
When facing a specific situation, humans can automatically distinguish the factors that may influence beliefs and trigger thoughts. Accordingly, we define the clue generation task as the flow ``\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-situation}\textit{Situation} $\Rightarrow$\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-clue}\textit{Clue}''. 
%Given a situation as input, \cokelm needs to predict the clues which determine the development of the cognitive chain. 

\textbf{Thought Generation}. 
In a specific situation, the related clues trigger and arouse diversified human mental activities, i.e., thoughts. Hereby, we define the thought generation task as the flow ``\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-situation}\textit{Situation} + \includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-clue}\textit{Clue} $\Rightarrow$\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-thought}\textit{Thought}''. 
%Given a situation and a clue as input, \cokelm needs to generate concrete human thoughts that act as the core in the cognitive chains.

\textbf{Action Generation}.
Driven by specific thoughts, we humans will take corresponding actions to realize our beliefs and achieve our goals. Thus we define the action generation task as the follow ``\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-situation}\textit{Situation}+\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-thought}\textit{Thought} $\Rightarrow$\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-action}\textit{Action}''. 
%Given a situation and a thought as input, \cokelm needs to predict the reasonable actions to characterize the behavioral response. 
Notice that we omit clues here since their impacts are largely covered by the triggered thoughts.

\textbf{Emotion Generation}.
After forming a specific thought in a certain situation, we humans will naturally generate corresponding emotions to express our attitudes and views on the situation. Therefore, we define the emotion generation task as the flow ``\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-situation}\textit{Situation} + \includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-thought}\textit{Thought} $\Rightarrow$\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-emotion-nomouse}\textit{Emotion} ''. 
%Given a situation and a thought as input, \cokelm needs to predict the emotion to characterize the affective response. 
Since emotions are limited to 6 categories, this task can be regarded as a classification task.

% The complete outputs of the above four tasks can be restored to cognitive chains"\textit{Situation {$\Rightarrow$} Clue {$\Rightarrow$} Thought {$\Rightarrow$} (Action$+$Emotion)}", 
By linking the above four tasks in a pipeline manner, we can restore the cognitive chain ``\textit{Situation {$\Rightarrow$} Clue {$\Rightarrow$} Thought {$\Rightarrow$} (Action$+$Emotion)}'', thus preserving the complete cognition process of ToM. Since each cognitive chain in \coke is labeled with polarity, each cognitive generation task can be further divided into positive and negative subtasks (e.g., positive thought generation and negative thought generation).


%.

\subsection{Training \cokelm}
%介绍特殊字符
After decomposing the cognitive chain into four cognitive generation tasks, we can process the data in \coke accordingly to obtain training samples for corresponding tasks. For computational efficiency, we design \cokelm as a multi-task controllable generation model, so that it can simultaneously accomplish four cognitive generative tasks and further control the polarity (i.e., positive or negative) of the outputs. As shown in Table \ref{tab-cokelm}, for each task and polarity, we insert specific tokens in the input $X$ to guide the generation process of \cokelm. For example, when training \cokelm for clue generation with a sample from negative cognitive chains, we append the special token \texttt{[NegClue]} to control \cokelm. For clarity, we only show one special token per type in Table \ref{tab-cokelm}. In practice, we use three special tokens like \texttt{[NegClue1]} \texttt{[NegClue2]} \texttt{[NegClue3]} per type for more stable control.

% After decomposing the cognitive chain into four cognitive generation tasks, we can process the data in \coke accordingly to obtain training samples for corresponding tasks. For computational efficiency, we design \cokelm as a multi-task controllable generation model, so that it can simultaneously accomplish four cognitive generative tasks and further control the polarity (i.e., positive or negative) of the outputs. For each task and polarity, we insert specific tokens to guide the generation process of \cokelm. \texttt{[Neg.*]} denotes special tokens for controllable generation in negative cognitive chains. When coming to positive cognitive chains, we use \texttt{[Pos.*]}. For example, when training \cokelm for clue generation with a sample from negative cognitive chains, we append the special token \texttt{[NegClue]} to control \cokelm. In practice, we use three special tokens like \texttt{[NegClue1]} \texttt{[NegClue2]} \texttt{[NegClue3]} per type for more stable control. More training details can be found in the \textit{Technical Appendix}.
%The input construction of other tasks can be found in Table \ref{tab-cokelm}, and more training details are present in Appendix X.


%介绍训练过程
For implementation, \cokelm is built as a standard encoder-decoder architecture and initialized with the pre-trained language model {T5-base} \cite{RaffelSRLNMZLL20}. Given an input-output pair $X$-$Y$ from any task, the encoder first transforms it into contextualized hidden representations. Then, at the $t$-th time step, the decoder takes the encoder's outputs and the previous decoding outputs $({y}_1,...,{y}_{t-1})$ as the input, and generates the next output token ${{y}}_{t}$.
In training, the encoder and decoder are jointly optimized to minimize the negative log-likelihood loss $\mathcal{L} = -\sum~_{t=1}^{n}l_t\cdot log(p({y}_{t}|X; {y}_{[1:t-1]}))$, where $l_t$ is the token label at position $t$ and $n$ is the length.






==> sections/05-experiment.tex <==
\section{Experiments}
\input{tables/automatic_evaluation4}
% 我们从 PLM中得到了原数据
% 在我们的知识图谱上 fine tune了T5  的到模型COKE+
% 
% 实验的目的： 是否可以帮助语言模型学习 ToM 的能力
% 做出的比较： 和InstructGPT 和 T5 做对比
In this section, we construct a dataset from \coke to evaluate the ToM ability of our cognitive generation model \cokelm, and compare it with T5-base (our backbone) and InstructGPT (our data source). We first illustrate the experimental setup, then analyze the experimental results for automatic and human evaluation, and finally validate \coke's effectiveness to empower social applications.


% We distilled the raw data from the InstructGPT \cite{Ouyang2022TrainingLM}, fine-tune the T5-{base}  model \cite{RaffelSRLNMZLL20} on our knowledge graph and got the \cokelm.  To evaluate whether our knowledge graph can help language models make cognitive inference efficiently, we compare the  \cokelm to the InstructGPT  and the pre-trained T5-{base}. The detailed testing and evaluation are described in this section.

% \begin{figure*}[h]
% 	% \centering
	
% 	\vspace{-6mm}
% 	\hspace{-10mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
% 	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
% 	% \includegraphics[width=0.85\linewidth]{figures/data_collection_cz}
%         \includegraphics[width=0.85\linewidth]{figures/esc_flow.png}
%         % \includegraphics{figures/data_collection.png}
% 	\centering
%         \caption{Empowering the ESC Model with \cokelm. A detailed case study is illustrated in the \textit{Technical Appendix}. }
% 	\label{fig-empowering}
% 	\vspace{-4mm}
% \end{figure*}

 
\subsection{Experimental Setup}
% 训练数据分布
    % 我们将数据分为训练集和测试集（）
        % 保证了测试集中每个话题的数量是均衡的
    % 在测试中模型需要做出 总共 6227 个节点的inference

% Baseline 模型
% 我们利用收集数据的任务描述 通过InstructGPT  对测试集进行推理。（Appendix E）
% 我们设计了prompt 以问答的形式 和 句子补全 的方式 引导 T5 对测试集推理。 （Appendix E）
% 最后将三个语言模型的结果进行对比。

% 训练模型的参数：
    % epoch batch size，  16
    % optimizer: AdamW
    % 运行设备： Tesla V100
    % GPU hours: about 9h



To evaluate the ToM ability of different models, we randomly split 1,200 social situations into 1,080 (90\%) training and 120 (10\%) validation situations. 
Then we can automatically split samples for different cognitive generation tasks according to the situations, and obtain training/validation splits as 19,409/2,268 (clue), 8,746/1,042 (thought), 17,982/1,893 (action), and 8,746/1,042 (emotion). Based on this setting, we ensure that the cognitive chains in the validation set all occur in \textbf{UNSEEN} situations, which is crucial for ToM evaluation. 

%We split 1200 social situations into training and test sets (90\% / 10\%), ensuring different topics in the test set are average.
%The models give 6227 inferences on the mode 
For \cokelm, we use the Hugging Face implementation\footnote{{https://huggingface.co/t5-base}.} of T5-{base}, and train it for 20 epochs using the AdamW optimizer \cite{LoshchilovH19} with learning rate 3e-4 and batch size 16 in a single Tesla V100 GPU. The whole training process costs about 9 GPU hours. For vanilla T5-base and InstructGPT, we construct manual prompts to enable them to complete the cognitive generation tasks.  More details can be found in the supplementary \textit{Technical Appendix}.The code can be found in the supplementary \textit{Code \& Data Appendix}. Due to the data deficiency, we report the performance on the validation set. 

% For \cokelm, we use the Hugging Face implementation\footnote{\href{https://huggingface.co/t5-base}{https://huggingface.co/t5-base}.} of T5-{base}, and train it for 20 epochs using the AdamW optimizer \cite{LoshchilovH19} with learning rate 3e-4 and batch size 16 in a single Tesla V100 GPU. The whole training process costs about 9 GPU hours. For vanilla T5-base and InstructGPT, we construct manual prompts to enable them to complete the cognitive generation tasks.  More details can be found in the supplementary \textit{Technical Appendix}.
% More details can be found in Appendix \ref{experiment-prompt}. 


%We compare our  \cokelm to the current most potent language model InstructGPT and T5-{base} model.



\subsection{Main Results}
% 实验数据
    % 运用了 BLEU和ACC
    % 一个输入有多个输出预测
    % 我们比较了多个输出的平均 BLEU score
%实验分析
    % COKE+ BLUE 分数都比GPT3高，除了 BLEU-2 Clue inference task 
    % 因为  InstructGPT 参数量就比COKE+高出5倍  并且 数据是从 InstructGPT 得到的
    % InstructGPT 在emotion classification 的任务上表现差的原因 ： 会做出wordy 的生成



\paragraph{Automatic Evaluation} To evaluate the clue/thought/action generation tasks, we use METEOR \cite{LavieD09}, ROUGE \cite{lin2004rouge}, BLEU-1, and BLEU-2 \cite{Papineni2002BleuAM} as metrics. In these three tasks, each input may be mapped to multiple ground truth outputs. 
%For example, in the clue generation task, a input situation can correspond to multiple output clues. 
Therefore, following \cite{mostafazadeh-etal-2020-glucose}, we compute the average  
%METEOR \cite{LavieD09}, ROUGE \cite{lin2004rouge}, BLEU-1 (Smoothing1), and BLEU-2 (Smoothing1) \cite{Papineni2002BleuAM} 
scores between all predicted sequences and all ground truth outputs\footnote{Here we provide all models with the required polarity (positive or negative) via special tokens or prompts.}. Moreover, to evaluate the emotion generation (classification) task, we compute the classification accuracy as the metric.
%We present the experimental results of clue/thought/action generation in Table \ref{tab-autoeval}. The accuracy scores for emotion generation are 0.3926 (T5-base), 0.4629 (InstructGPT), and 0.7598 (\cokelm), which have been omitted in Table \ref{tab-autoeval} for convenience.
%We present the automatic evaluation results of clue/thought/action generation in the first four rows of Table \ref{tab-autoeval}. The accuracy scores for emotion generation, which are 0.3926 (T5-base), 0.4629 (InstructGPT), and 0.7598 (\cokelm), have been omitted in the table for the sake of convenience.
We present the automatic evaluation results of clue/thought/action generation in the first four rows of Table \ref{tab-autoeval}. For clarity, the accuracy scores for emotion generation are included in the table caption.

Compared to the backbone T5-base, \cokelm exhibits a large performance boost for cognitive generation tasks of ToM. Compared to the powerful InstructGPT which is about 800 times larger (175B v.s. 220M), \cokelm still shows significant advantages in most evaluation metrics. We hereby have two observations: 1) The data we collected in \coke is of high quality and can empower the model with strong ToM ability. 2) \cokelm, which is designed as a controllable generative model for multiple cognitive tasks, can effectively internalize the ToM ability and cope with unseen situations.% after being trained on \coke.


\paragraph{Human Evaluation} Beyond automatic evaluation, we also wonder how humans perceive the cognitive chains generated by different models since ToM is essentially a human ability. Therefore, for each model, we sample a cognitive chain for each situation in the validation set (resulting in a total of 120 samples per model) for human evaluation. We present three experts with the cognitive chains generated by different models and then ask them to score them on a 3-point Likert scale: ``completely incorrect (1 point)'', ``almost correct (2 point)'', and ``completely correct (3 point)''. The averaged scores over three experts and 120 samples are used to evaluate the model's ToM ability. The results in the last row of Table \ref{tab-autoeval} demonstrate that the cognitive chains generated by \cokelm are more acceptable to humans, which again shows the superiority of its ToM ability. We further present ten cognitive chains generated by \cokelm in five situations covering different topics in the supplementary \textit{Technical Appendix}.


%the model trained on our knowledge graph has better cognitive inference than the InstructGPT, whose parameters are five times more than  \cokelm. Compared to the powerful InstructGPT, which generates the raw data, our model has better BLEU scores except for the BLUE-2 score of the clue inference task.

 %and the emotion generation (can be viewed as classification) using the Accuracy score.
 
\begin{comment}

For automatic evaluation, we evaluate the clue/thought/action generation tasks using the BLEU scores \cite{Papineni2002BleuAM}. For the above three task, each input may be mapped to multiple gold outputs. For example, the situation as the input in the clue inference task typically has more than two target clues in \coke. We compute the average BLEU-1 (Smoothing1) score and BLEU-2 score (Smoothing1) \cite{Papineni2002BleuAM} between all predicted sequences and the corresponding set of \coke. Table \ref{tab-autoeval} presents the result on the TEST dataset. The experiments show that the model trained on our knowledge graph has better cognitive inference than the InstructGPT, whose parameters are five times more than  \cokelm. Compared to the powerful InstructGPT, which generates the raw data, our model has better BLEU scores except for the BLUE-2 score of the clue inference task.
\end{comment}



% \subsection{Human Evaluation}
% Beyond automatic evaluation, we also wonder how humans perceive the cognitive chains generated by different models since ToM is essentially a human ability. Therefore, for each model, we sample a cognitive chain for each situation in the validation set (resulting in a total of 120 samples per model) for human evaluation. We present three experts with the cognitive chains generated by different models and then ask them to score them on a three-point Likert scale: ``completely incorrect (1 point)'', ``almost correct (2 points)'', and ``completely correct (3 points)''. The averaged scores over three experts and 120 samples are used to evaluate the model's ToM ability. The results in Table \ref{tab-humanevaluation} demonstrate that the cognitive chains generated by \cokelm are more acceptable to humans, which again shows the superiority of its ToM ability. Due to the space limitation, we present ten cognitive chains generated by \cokelm in five situations covering different topics in Appendix \ref{appendix-casestudy}. 
% \input{tables/human_evaluation.tex}

%\subsection{Benefits of \coke for ToM-Based Social Applications}
\subsection{Empowering Social Applications with \coke}
As \coke is a cognitive knowledge graph for machine theory of mind, we further substantiate its effectiveness in empowering social applications with ToM capabilities. 
Our chosen testing ground is the Emotional Support Conversation (ESC) task \cite{DBLP:conf/acl/LiuZDSLYJH20}. The prime objective of ESC is to generate empathetic and effective responses in social dialogues, with the aim of mitigating users' emotional distress and fostering improved mental states. ESC requires ToM because it involves understanding and responding to a user's emotional state and underlying challenges, which necessitates an understanding of their mental processes and intentions.





% ESC is an ideal testing ground for demonstrating the potency of \coke as it necessitates a deep comprehension of and responsiveness to a user's emotional state and the underlying challenges they may be facing. This understanding transcends the surface level, requiring insight into the user's mental processes and intentions. Furthermore, providing effective comfort and suggestions is contingent on the ability to anticipate the user's emotional trajectory and potential reactions to varied forms of support. This ability to infer and respond in an empathetic manner is a cornerstone of ToM.

%Additionally, the ability to offer effective comfort and suggestions hinges on the capacity to infer the user's emotional trajectory and potential reactions to different forms of support.


\paragraph{Integration of \coke in ESC}

As shown in Figure \ref{fig-empowering}, the ESC dataset has already provided the {situation} behind each dialogue. We then treat each user's utterance in the dialogue as a {clue}, and employ \cokelm to infer two thoughts (1 positive and 1 negative) via thought generation (\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-situation}\textit{Situation} + \includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-clue}\textit{Clue} $\Rightarrow$\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-thought}\textit{Thought}). Based on the generated thoughts, we can accordingly infer
% three 
actions for each thought via action generation (\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-situation}\textit{Situation}+\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-thought}\textit{Thought} $\Rightarrow$\includegraphics[height=1em,trim=0 3em 0 0]{figures/openmoji-action}\textit{Action}). We simply extract verbs and nouns in thoughts or actions as the ToM knowledge keywords, and append them to the end of dialogue history, serving as an enhanced context. Based on the context, the ESC system is trained to generate the corresponding response. We here use the Blenderbot \cite{DBLP:conf/eacl/RollerDGJWLXOSB21} as the generation model, which is the same as the original ESC paper \cite{DBLP:conf/acl/LiuZDSLYJH20}. 

\begin{figure*}[h]
	\centering
	\vspace{1mm}
	\hspace{-2mm}
	\setlength{\abovecaptionskip}{0mm}
	\setlength{\belowcaptionskip}{0mm}
	%\includegraphics[width=0.98\linewidth]{figures/data_collection.png}
	% \includegraphics[width=0.85\linewidth]{figures/data_collection_cz}
        \includegraphics[width=0.98\linewidth]{figures/esc_flow.png}
         % \includegraphics[width=0.85\linewidth]{figures/esc_flow_wider.png}
        % \includegraphics{figures/data_collection.png}
	\centering
        \caption{Empowering ESC with \cokelm. A detailed case study is illustrated in the \textit{Technical Appendix}. }
	\label{fig-empowering}
	\vspace{-2mm}
\end{figure*}




%\paragraph{Experimental Results of ESC}
\paragraph{ESC Performance with ToM Knowledge}
% \input{tables/AppendixH_Example}
% In our experiments, we compare three models: Vanilla ESC, ESC with \cokelm Actions, and ESC with \cokelm Thoughts. Both automatic (PPL, BLEU-2, ROUGE-L, Extrema) and human (Fluency, Identification, Comforting, Suggestion) evaluations are conducted, following the same methodology as the original ESC paper. The results of these evaluations are presented in Table \ref{tab-esc-autoevaluation}.
% The experimental results demonstrate that, when incorporating the ToM knowledge into the response generation process, both the ESC with \cokelm Actions and ESC with \cokelm Thoughts models significantly outperform the Vanilla ESC model across all metrics. The results demonstrate the potential of \coke to empower social applications, offering a more nuanced and empathetic approach to AI-driven emotional support. By integrating \coke's cognitive chains into dialogue history, AI systems can achieve a more sophisticated understanding of human emotions and behavior, leading to more effective interactions in emotionally charged contexts such as the ESC task. Interestingly, the ESC with \cokelm Thoughts model shows a slight advantage over the ESC with \cokelm Actions model. This could be attributed to the fact that the thoughts generated by \cokelm offer a more direct reflection of the user's mental state.


In our experiments, we compare three models: Vanilla ESC, ESC with \cokelm Actions, and ESC with \cokelm Thoughts. Both automatic and human  evaluations are conducted, following the same methodology as the original ESC paper. The results of these evaluations are presented in Table \ref{tab-esc-autoevaluation}.
The experimental results demonstrate that, when incorporating the ToM knowledge into the response generation process, both the ESC with \cokelm Actions and ESC with \cokelm Thoughts models significantly outperform the Vanilla ESC model across all metrics. The results demonstrate the potential of \coke to empower social applications, offering a more nuanced and empathetic approach to AI-driven emotional support. By integrating \coke's cognitive chains into dialogue history, AI systems can achieve a more sophisticated understanding of human emotions and behavior, leading to more effective interactions in emotionally charged contexts such as the ESC task. Interestingly, the ESC with \cokelm Thoughts model shows a slight advantage over the ESC with \cokelm Actions model. This could be attributed to the fact that the thoughts generated by \cokelm offer a more direct reflection of the user's mental state.
\input{tables/AppendixH_ESC_AE}


% To delve deeper into the performance of these models, we also present a case study in Appendix\ref{appendix-esc}. This sample highlights a conversation between the system and a user who is struggling with feelings of loneliness and a lack of friends. The Vanilla ESC model, however, generates a response that is somewhat disjointed and lacks clear relevance to the user's situation. It mentions popular apps and sites like "facetime", but doesn't connect this suggestion to the user's problem (lack of friends). Thus, it fails to show an understanding of the user's feelings or provide a relevant solution. While for ESC w/ \cokelm Thoughts, the identified ToM keywords encapsulate the user's emotional state (\textit{negative}), their sense of isolation (\textit{alone}), their need (\textit{make friends}), and their perceived challenge (\textit{confront something}). Therefore, the empowered ESC model provides a response that aligns much better with the user's emotional state and context. This response directly addresses the user's unfamiliarity with friendship apps, explaining their purpose in a straightforward and reassuring manner. It further expands on the concept by highlighting the potential for meeting people from different cultures, implying a broad range of possible connections that could enrich the user's social experience.

% Due to the space limitation, we present the detailed conversation in the supplementary \texttt{Technical Appendix}.
% \ref{appendix-casestudy}. 

% \input{tables/AppendixH_Example}



% To delve deeper into the performance of these models, we also present a case study in Table \ref{tab-esc-case}. This sample highlights a conversation between the system and a user who is struggling with feelings of loneliness and a lack of friends. The Vanilla ESC model, however, generates a response that is somewhat disjointed and lacks clear relevance to the user's situation. It mentions popular apps and sites like "facetime", but doesn't connect this suggestion to the user's problem (lack of friends). Thus, it fails to show an understanding of the user's feelings or provide a relevant solution. 

% While for ESC w/ \cokelm Thoughts, the identified ToM keywords encapsulate the user's emotional state (\textit{negative}), their sense of isolation (\textit{alone}), their need (\textit{make friends}), and their perceived challenge (\textit{confront something}). Therefore, the empowered ESC model provides a response that aligns much better with the user's emotional state and context. This response directly addresses the user's unfamiliarity with friendship apps, explaining their purpose in a straightforward and reassuring manner. It further expands on the concept by highlighting the potential for meeting people from different cultures, implying a broad range of possible connections that could enrich the user's social experience.

% Details and results can be found in Appendix \ref{appendix-esc}.
% The experimental results provide compelling evidence of the impact of integrating \coke into the ESC task. Upon the introduction of the cognitive knowledge derived from \coke, there is a significant improvement in the performance of the ESC system, validated by both automatic and human evaluation. To uphold the principles of accountability, transparency, and fairness, we additionally include an ethics statement about \coke in Appendix \ref{appendix-ethics}. 


 
 % ESC requires Theory of Mind (ToM) because it involves understanding and responding to a user's emotional state and underlying challenges, which necessitates an understanding of their mental processes and intentions. Additionally, the ability to offer effective comfort and suggestions hinges on the capacity to infer the user's emotional trajectory and potential reactions to different forms of support, a capability central to ToM. The experimental results demonstrate that, after introducing knowledge from \coke, the ESC system performs significantly better on both automatic and human metrics. 

%We opt to test this in a task that fundamentally requires ToM: Emotional Support Conversation (ESC) \cite{DBLP:conf/acl/LiuZDSLYJH20}. The goal of ESC is to generate responses in dialogues to alleviate users' emotional distress and improve their mental states.  The Emotional Support Conversation (ESC) task requires Theory of Mind (ToM) because it involves understanding and responding to a user's emotional state and underlying challenges, which necessitates an understanding of their mental processes and intentions. Additionally, the ability to offer effective comfort and suggestions hinges on the capacity to infer the user's emotional trajectory and potential reactions to different forms of support, a capability central to ToM.




% 为什么做人工实验
%Since the automatic evaluation of generation work has been a significant bottleneck for research, we also assess our models’ performance through human evaluation.
%人工实验的数据
    % 一个场景中有多条 cognitive chain 
    % 我们每个场景选择其中一条chain. 
    % 每个任务只做一条推理。 

%We randomly select one cognitive chain from the test dataset for each situation and generate one inference per dimension.


%评估的标准
    % 我们将所有结果给两位 experts 打分 并以均值作为 评估标准
    % 对于每一个生成任务
        % expert 先看对应的输入
        % 再评估测试结果
        % 为测试结果打 0-2分分别对应  不正确/勉强正确/ 完全正确。     
            %===============（用正确这个词是否合适， 是否需要换成 likely/reasonable）==========
        % 为了帮助expert 打分，我们提供test set 的gold data 去帮助 区分 勉强正确和完全正确
        
%We set up the following evaluation process to ensure calibrated judgments. We present two experts with all generated inferences and get averaged scores.
%For each generation task, the expert first reads the input, then checks the validity of candidate inferences. The judge rates each candidate inferences on a three-point Likert scale: "completely incorrect," "almost correct," and " completely correct. " The ratings are mapped to numerical scores of 0-2, which are then averaged to compare model performance.


%评分的分析
    % InstructGPT 表现不好的原因
        % 会生成很冗长的内容 容易生成 勉强正确的答案
    % T5的表现很差的原因
        % ToM相关的任务，对于T5 来说太陌生
        % 对于容易生成和任务不相关的句子 做出完全错误的回答
%The powerful InstructGPT does not give an impressive performance since it is often excessively verbose and generates almost correct inferences. T5-{base}  poor performance shows that finetuning on our knowledge graph significantly improves the Theory of Mind inference capabilities of language models.


\begin{comment}

\subsection{Case Study}
% 突出是unseen situations
To have a close look, we further collect ten cognitive chains generated by \cokelm in \textbf{unseen} situations in a pipeline manner. As shown in Table \ref{tab-case_study}, the selected ten cognitive chains cover all five topics and both positive and negative polarities. It can be seen that for the same situation, \cokelm can generate positive and negative cognitive chains, and effectively characterize the human mental state and cognitive process. Therefore, we can claim that \cokelm has the basic ToM ability to understand humans' desires, beliefs, and intentions.


%We present sample Theory of Mind inferences predictions in .
%We give negative and positive cognitive chains of five situations in different topics.

\input{tables/case_study.tex}

\end{comment}

% \begin{figure*}[t]
% 	\centering
% 	\vspace{0mm}
% 	\hspace{0mm}
% 	\setlength{\abovecaptionskip}{1mm}
% 	\setlength{\belowcaptionskip}{1mm}
%         \includegraphics[width=1\textwidth]{figures/case_study.png}
% 	\centering
% 	\caption{Cases in five topics }
% 	\label{fig-case_study}
% 	\vspace{-5mm}
% \end{figure*}

==> sections/06-conclusion.tex <==
\section{Conclusion}
\vspace{1.5mm}
In this work, we present \cokewithemoji, the first cognitive knowledge graph for machine theory of mind. We instantiate ToM as a series of cognitive chains to describe human mental activities and behavioral/affective responses in social situations.
Through prompting InstructGPT and manual annotation, we collect 62k+ nodes and construct 45k+ cognitive chains.
Based on \coke, we build a powerful cognitive generation model \cokelm. \cokelm can handle unseen situations and predict complete cognitive chains in a pipeline manner. Automatic and human evaluations show that \cokelm effectively internalizes the ToM ability and outperforms strong baseline models like InstructGPT. We believe this work demonstrates a viable path to advance AI systems and enable them to serve humanity better.
In the future, we will keep increasing the size of the cognitive knowledge graph and enhance the performance of the cognitive generation model, and further apply them to downstream NLP tasks, including affective computing and dialogue systems.






==> sections/07-limitation.tex <==

\section*{Limitations}
In this work, we introduce \cokewithemoji, the first cognitive knowledge graph for machine Theory of Mind, which aims to empower AI systems with cognitive capabilities. However, we acknowledge the following omissions and inadequacies in our work.
\paragraph{Data Coverage}
We acknowledge that there is a limitation in topic coverage of proposed \cokewithemoji, which only covers five social topics that are commonly discussed.
Besides, \cokewithemoji has a relatively small data scale in comparison with other relative knowledge graphs, due to its more specific node contents and more complicated construction process.
Consequently, \cokewithemoji cannot cover all situations in deployment, and the cognitive reasoning models constructed on this basis may have unreliable predictions in out-of-domain situations.
\paragraph{Cognitive Inference Ability}
As a pioneer in integrating \emph{Theory of Mind} into AI systems, the proposed cognitive generation model \cokelm still has a lot of room for improvement in inferring cognitive chains when deployed in practice.
In \cokelm, we take T5-base as the backbone model to validate the gain of \cokewithemoji on the cognitive inference ability of language models.
We acknowledge that adopting larger backbone models  would contribute to a more powerful inference model, which is worth exploring in more depth in the future.
\paragraph{Exploration in Downstream Tasks}
This work did not validate the gain of \cokewithemoji for downstream tasks.
We believe that incorporating this knowledge into downstream tasks, such as emotion recognition and empathetic response generation, would lead to significant gains. We call for more work in this direction.

\section*{Ethics Statement}
% \paragraph{Data Usage}
We present the first cognitive knowledge graph \cokewithemoji for machine theory of mind.
Our knowledge graph is built based on public datasets and model generations.
We strictly adhere to data source usage protocols and ensure that the proposed \cokewithemoji can be released and used \MakeUppercase{legally}.

The construction of \cokewithemoji has gone through the steps of manual selection and revision.
We manually filtered the data containing potentially private information, such as phone numbers and email addresses, to protect user \MakeUppercase{privacy} further. 
We also carefully delete abusive, offensive, biased, and other inappropriate content to avoid unpredictable \MakeUppercase{ethical} hazards.

% \paragraph{Potential Misuse}
Our knowledge graph is designed to empower AI systems with the ability of cognitive inference.
We are aware that this capability could be misused in malicious scenarios in the future. However, we believe the value of this work outweighs the risks, and we also call for more socially responsible research in this field.

==> tables/automatic_evaluation.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% \textbf{Model} & \textbf{Clue BLEU-1} & \textbf{Thought BLEU-1} & \textbf{Action BLEU-1} & \textbf{Clue BLEU-2} & \textbf{Thought BLEU-2} & \textbf{Action BLEU-2} & \textbf{Emotion Accuracy} \\ \midrule
% T5 Base        & 0.119                & 0.1537                  & 0.1382                 & 0.0036               & 0.0143                  & 0.0091                 & 0.39                      \\
% InstructGPT    & 0.1428               & 0.2872                  & 0.3138                 & \textbf{0.0222}      & 0.0279                  & 0.0044                 & 0.46                      \\
% \cokelm          & \textbf{0.3378}      & \textbf{0.3883}         & \textbf{0.376}         & 0.0114               & \textbf{0.0389}         & \textbf{0.0268}        & 0.76                      \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}


\begin{table*}[h]
\vspace{0mm}
\small
%\scriptsize
%\footnotesize
\renewcommand\arraystretch{1.05}
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{1mm}
\centering
\setlength{\tabcolsep}{1.0mm}

\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Model} & \textbf{Clue BLEU-1/BLEU-2} & \textbf{Thought BLEU-1/BLEU-2} & \textbf{Action BLEU-1/BLEU-2} & \textbf{Emotion Accuracy} \\ \midrule
T5-base    & 0.1190/0.0036           & 0.1537/0.0143          & 0.1382/0.0091         & 0.39          \\
InstructGPT & 0.1428/\textbf{0.0222}          & 0.2872/0.0279          & 0.3138/0.0044         & 0.46          \\
\cokelm       & \textbf{0.3378}/0.0114 & \textbf{0.3883/0.0389} & \textbf{0.376/0.0268} & \textbf{0.76} \\ \bottomrule

\end{tabular}

\caption{Automatic evaluation results for models.BLEU scores are out of 100.}
\label{tab-autoevaluation}
\vspace{0mm}
\end{table*}



==> tables/automatic_evaluation2.tex <==

% ============== Version 2 ==============

\begin{table}[h]
\centering
\small
\vspace{2mm}
\renewcommand\arraystretch{1.3}
\setlength{\abovecaptionskip}{3mm}
\setlength{\belowcaptionskip}{3mm}
\setlength{\tabcolsep}{1.0mm}
\begin{tabular}{c|c|ccc}
\hline
\multirow{2}{*}{Task}         & \multirow{2}{*}{Metric} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}T5-base\\ (220M)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}InstructGPT\\ (175B)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\cokelm\\ (220M)\end{tabular}} \\
    &   &   &    &  \\ \hline
\multirow{2}{*}{Clue Gen.}    
& BLEU-1  & 0.1190  & 0.1428  & \textbf{0.3378}$^{\dagger}$                                                                  \\
 & BLEU-2    & 0.0036   & \textbf{0.0222}    & 0.0114$^{~}$                                                                 \\ \hline
\multirow{2}{*}{Thought Gen.} 
& BLEU-1   & 0.1537   & 0.2872  & \textbf{0.3883}$^{\dagger}$    \\
& BLEU-2   & 0.0143  & 0.0279     & \textbf{0.0389}$^{\dagger}$    \\ \hline
\multirow{2}{*}{Action Gen.}  
& BLEU-1    & 0.1382   & 0.3138  & \textbf{0.3760}$^{\dagger}$  \\
& BLEU-2    & 0.0091   & 0.0044  & \textbf{0.0268}$^{\dagger}$   \\ \hline
Emotion Gen.                  
& Acc.   & 0.3926  & 0.4629  & \textbf{0.7598}$^{\dagger}$                                                                 \\ \hline
\end{tabular}
\caption{Automatic evaluation results for all cognitive generation tasks. The highest scores are in bold. All results are average scores of 3 runs with random seeds, and those with ${\dagger}$ are significantly better than baselines with $p<0.01$. We also present the parameter number below each model.}
\label{tab-autoeval}
\vspace{-6mm}
\end{table}

\begin{comment}
\begin{tabular}{c|c||ccc} 
%\toprule
\hline
%\multicolumn{2}{l}{Model}   
%\multicolumn{2}{l}{\diagbox{Task}{Model}}  
% & Model 
\multirow{2}{*}{Task} &\multirow{2}{*}{ Metric} & \multirow{2}{*}{T5-{base}} & \multirow{2}{*}{InstructGPT} & \multirow{2}{*}{\cokelm}   \\ 
\\
\hline
%\midrule
\multirow{2}{*}{Clue Gen.}    & BLEU-1   & 0.1190  & 0.1428      & \textbf{0.3378}  \\
                         & BLEU-2   & 0.0036  & \textbf{0.0222}      & 0.0114  \\ 
%\midrule 
\hline
\multirow{2}{*}{Thought Gen.} & BLEU-1   & 0.1537  & 0.2872      & \textbf{0.3883}  \\
                         & BLEU-2   & 0.0143  & 0.0279      & \textbf{0.0389}  \\ 
%\midrule
\hline
\multirow{2}{*}{Action Gen.}  & BLEU-1   & 0.1382  & 0.3138      & \textbf{0.3760}   \\
                         & BLEU-2   & 0.0091  & 0.0044      & \textbf{0.0268}  \\ 
%\midrule
\hline
Emotion Gen.                  & Acc. & 0.3926    & 0.4629        & \textbf{0.7598}    \\
%\bottomrule
\hline
\end{tabular}

\end{comment}

==> tables/automatic_evaluation3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\small
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{1mm}
\resizebox{0.70\textwidth}{!}{%
\begin{tabular}{llllllll}
\hline
\multicolumn{1}{c}{Model} &
  \multicolumn{1}{c}{Meteor} &
  \multicolumn{1}{c}{PPL} &
  \multicolumn{1}{c}{Rouge} &
  % \multicolumn{1}{c}{Distinct} &
  \multicolumn{1}{c}{BLUE-1} &
  \multicolumn{1}{c}{BLEU-2} &
  \multicolumn{1}{c}{ACC} \\ \hline
  
% T5-base (220M)     & 0.1653 & 147.94         & 0.1192 & \textbf{0.8937} & 0.137  & 0.009  & 0.3928 \\
% InstructGPT (175B) & 0.2361          & \textbf{32.29} & 0.1475          & 0.8466          & 0.2479          & 0.0182          & 0.4629          \\
% COKE+(220M)        & \textbf{0.2888} & 59.03          & \textbf{0.2657} & \textbf{0.8385} & \textbf{0.3673} & \textbf{0.0257} & \textbf{0.7598} \\ 
T5-base (220M)     & 0.1653 & 147.94         & 0.1192 & 0.1370  & 0.009  & 0.3928 \\
InstructGPT (175B) & 0.2361          & \textbf{32.29} & 0.1475          &  0.2479          & 0.0182          & 0.4629          \\
\cokelm(220M)        & \textbf{0.2888} & 59.03          & \textbf{0.2657} &  \textbf{0.3673} & \textbf{0.0257} & \textbf{0.7598} \\ 



\hline
\end{tabular}%
}
\caption{Automatic evaluation results for all cognitive generation tasks. The highest scores are in bold. All results are average scores of 3 runs with random seeds, and those with ${\dagger}$ are significantly better than baselines with $p<0.01$. We also present the parameter number below each model.}
\label{tab-autoeval}
\vspace{-6mm}
\end{table}

==> tables/dimension.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

% \begin{table*}[t]
% \centering
% \scalebox{0.74}{
% \begin{tabularx}{1.3\textwidth}{
%     m{.10\textwidth}
%     m{.26\textwidth} 
%     m{.22\textwidth} 
%     m{.39\textwidth}
%     m{.21\textwidth}} 
% \toprule
% \multicolumn{5}{c}{\textbf{Situation: I enter the waiting room for the interview.}}                                                                                                                                                                                                                                                                                                 \\ \midrule
% \textbf{Dimension}       & \textbf{Definition}   & \textbf{Class}          & \textbf{Definition}                                            \\ \midrule
% \multirow{4}{*}{Clue}    & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}
%                          \\the knowledge related to\\ situations trigger various\\ cognitive responses\end{tabular}} & Other Clue  & Particular information about the others’ appearance, actions, personality, etc. \\ \cmidrule{3-5} 
%                          &                                                                                           & Social Clue & Particular information about how people behave in social situations       \\ \cmidrule{3-5} 
%                          &                                                                                           & Object Clue & How people comprehend what various items are, how they should work, and etc.  \\ \cmidrule{3-5} 
%                          &                                                                                           & Person Clue & Particular information about our appearance, actions, personality, etc \\ \midrule
% \multirow{2}{*}{Thought} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}the mental state that \\ affects emotion and \\ behaviors directly\end{tabular}}               
%                                                                                                                     & Negative Thought &                   \\ \cmidrule{3-5} 
%                          &                                                                                          & Positive Thought &                    \\ \midrule
% \multirow{2}{*}{Emotion} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}describes the feelings evo-\\ked by specific thought\end{tabular}}                                                                 & Angry/ Sad/ Fearful,    & Negative Emotion                                                                                              & Sad                                                      \\ \cmidrule{3-5} 
%                          &                                                                                                                                        & Joyful/ Love/ Surprised & Positive  Emotion                                                                                                           & Joyful                                                   \\ \midrule
% \multirow{3}{*}{Action}  & \multirow{3}{*}{Behavioral Response}                                                                                                   & \multirow{3}{*}{}       &                                                                                                                                            \\ \cmidrule{4-5} 
%                          &                                                                                                                                        &                         &                                                                                                                                        \\ \cmidrule{4-5} 
%                          &                                                                                                                                        &                         &                                                                                                                                        \\ \bottomrule
% \end{tabularx}
% }
% \end{table*}

% \begin{table*}[t]
% \centering
% \scalebox{0.74}{
% \begin{tabularx}{1.3\textwidth}{
%     m{.10\textwidth}
%     m{.26\textwidth} 
%     m{.22\textwidth} 
%     m{.39\textwidth}
%     m{.21\textwidth}} 
% \toprule
% \multicolumn{5}{c}{\textbf{Situation: I enter the waiting room for the interview.}}                                                                                                                                                                                                                                                                                                 \\ \midrule
% \textbf{Dimension}       & \textbf{Definition}   & \textbf{Class}          & \textbf{Definition}    & \textbf{Examples}                                        \\ \midrule
% \multirow{4}{*}{Clue}    & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\\the knowledge  related to\\ situations trigger various\\ cognitive responses\end{tabular}} & Other   Clue            
%                          & Particular   information about the others’ appearance, actions, personality, etc & The secretary does not let me sign in.                   \\ \cmidrule{3-5} 
%                          &                                                                                                                                        & Social Clue    
%                          & Particular information about how people behave in social situations
%                          % & \begin{tabular}[c]{@{}l@{}}Particular   information about how\\ people behave in social situations\end{tabular}             
%                          & Too many   people interview for the job.                 \\ \cmidrule{3-5} 
%                          &                                                                                                                                        & Object Clue             & How people comprehend what various items are, how they should work, and etc       & It is a   public traded company.                         \\ \cmidrule{3-5} 
%                          &                                                                                                                                        & Person Clue             & Particular information about our appearance, actions, personality,etc            & I have   10 years of experience in this field.           \\ \midrule
% \multirow{2}{*}{Thought} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}the mental state that \\ affects emotion and \\ behaviors directly\end{tabular}}               & Negative Thought        &                                                                                                                             & I will   not be selected.                                \\ \cmidrule{3-5} 
%                          &                                                                                                                                        & Positive Thought        &                                                                                                                             & I will   have a good career after joining in the company \\ \midrule
% \multirow{2}{*}{Emotion} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}describes the feelings evo-\\ked by specific thought\end{tabular}}                                                                 & Angry/ Sad/ Fearful,    & Negative Emotion                                                                                                            & Sad                                                      \\ \cmidrule{3-5} 
%                          &                                                                                                                                        & Joyful/ Love/ Surprised & Positive  Emotion                                                                                                           & Joyful                                                   \\ \midrule
% \multirow{3}{*}{Action}  & \multirow{3}{*}{Behavioral Response}                                                                                                   & \multirow{3}{*}{}       &                                                                                                                             & find a   staff to complete the sign-in                   \\ \cmidrule{4-5} 
%                          &                                                                                                                                        &                         &                                                                                                                             & go over   the answers to interview questions.            \\ \cmidrule{4-5} 
%                          &                                                                                                                                        &                         &                                                                                                                             & talk to   the other candidates confidently.              \\ \bottomrule
% \end{tabularx}
% }
% \end{table*}

\begin{comment}
\begin{table*}[h]
\vspace{0mm}
\small
%\scriptsize
%\footnotesize
\renewcommand\arraystretch{1.05}
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{1mm}
\centering
\setlength{\tabcolsep}{1.0mm}

\begin{tabular}
{@{}cccc@{}}
\toprule
\textbf{Dimension} &
  \textbf{Definition} &
  \textbf{Class} &
  \multicolumn{1}{c}{\textbf{Class Details}} \\ \midrule   
  \multirow{4}{*}{Clue} &
  \multirow{4}{*}{ \makecell[l]{The information related to situations\\concretizes and differentiates thoughts }} &  Person Clue & \makecell[l]{Particular information about our\\appearance, personality, etc.}   \\ \cmidrule(l){3-4} &  
                                                                                                                &  Other Clue & \makecell[l]{Particular information about the others’\\appearance, actions, personality, etc.}   \\ \cmidrule(l){3-4} & 
                                                                                                                &Social Clue & \makecell[l]{Particular information about\\how people behave in social situations}   \\ \cmidrule(l){3-4} &
                                                                                                                &  Object Clue & \makecell[l]{How people comprehend what various\\items are, how they should work, etc.}   \\ \midrule
\multirow{2}{*}{Thought} &\multirow{2}{*}{The cognitive response to the situation}
&Negative Thought &The thought triggers negative   emotions. \\ \cmidrule(l){3-4} &
&Positive Thought &The thought triggers positive   emotions. \\ \midrule
\multirow{2}{*}{Emotion} &\multirow{2}{*}{  \makecell[l]{The affective response to the situation\\with the specific thought } } &
  Negative Emotion &
  Angry, Sad, Fearful \\ \cmidrule(l){3-4} &&
  Positive Emotion &Joyful, Love, Surprised \\ \midrule
  Action &      \makecell[l]{The behavioral response to the\\situation with the specific thought}    & &
   \\ \bottomrule

\end{tabular}

\caption{The dimension of the knowledge graph.}
\label{tab-dimension}
\vspace{0mm}
\end{table*}
\end{comment}






\begin{comment}


\begin{table}[h]
\vspace{0mm}
\small
%\scriptsize
%\footnotesize
\renewcommand\arraystretch{1.05}
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{1mm}
\centering
\setlength{\tabcolsep}{1.0mm}

\begin{tabular}{}

\end{tabular}

\caption{The statistics of datasets.}
\label{tab-dataset}
\vspace{0mm}
\end{table}


\end{comment}

\begin{table*}[h]
\vspace{0mm}
\small
%\scriptsize
%\footnotesize
\renewcommand\arraystretch{1.2}
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{1mm}
\centering
\setlength{\tabcolsep}{0.3mm}


\begin{tabular}{l|l|l}
	\hline
	\multicolumn{1}{c|}{\textbf{Node}}       &\multicolumn{1}{c|}{\textbf{Definition}}    &\multicolumn{1}{c}{\textbf{Example}}       \\ 
	\hline
	\emojisituation{Situation} 
	& \tabincell{l}{The social circumstances that the subject (potentially) \\interacts with other individuals.} 
	& \textit{I shall deliver a speech at the university tomorrow.}  \\ 
	\hline
	\emojiclue{Clue}      
	& The factors that trigger and concretize thoughts.   
	& \tabincell{l}{ \texttt{Positive} | \textit{I have substantial public speaking experience.}\\ \texttt{Negative} |  \textit{There may be many audiences.}} \\ 
	\hline
	\emojithought{Thought}   
	& \tabincell{l}{The beliefs and intentions acting as the cognitive\\responses to the situations.}   
	& \tabincell{l}{ \texttt{Positive} | \textit{I will deliver an impressive speech.}\\ \texttt{Negative} | \textit{I may mess up the speech.}}  \\ 
	\hline	
	\emojiaction{Action}   
	& \tabincell{l}{The behavioral responses to the situations with\\the specific thoughts.}                   
	& \tabincell{l}{ \texttt{Positive} | \textit{I have a restful sleep tonight.}\\ \texttt{Negative} | \textit{I practice my script in front of the mirror.}} \\ 
	\hline
	\emojiemotion{Emotion}   
	& \tabincell{l}{The affective responses to the situations with\\the specific thoughts.}                       
	& \tabincell{l}{ \texttt{Positive} | \textit{Joyful}\\ \texttt{Negative} | \textit{Fearful}}                                                             \\ \hline
\end{tabular}
\caption{The node definition in the cognitive knowledge graph \coke. The prefixes \texttt{Positive} and \texttt{Negative} indicate that the example nodes are sampled from positive and negative cognitive chains, respectively. }
\label{tab-dimension}
\vspace{0mm}
\end{table*}
